(Nearly) Sample-Optimal Sparse Fourier Transform in Any Dimension; RIPless and Filterless

In this paper, we consider the extensively studied problem of computing a $k$-sparse approximation to the $d$-dimensional Fourier transform of a length $n$ signal. Our algorithm uses $O(k \log k \log n)$ samples, is dimension-free, operates for any universe size, and achieves the strongest $\ell_\infty/\ell_2$ guarantee, while running in a time comparable to the Fast Fourier Transform. In contrast to previous algorithms which proceed either via the Restricted Isometry Property or via filter functions, our approach offers a fresh perspective to the sparse Fourier Transform problem.

==> arxiv/abstract.tex <==
In this paper, we consider the extensively studied problem of computing a $k$-sparse approximation to the $d$-dimensional Fourier transform of a length $n$ signal. Our algorithm uses $O(k \log k \log n)$ samples, is dimension-free, operates for any universe size, and achieves the strongest $\ell_{\infty}/\ell_2$ guarantee, while running in a time comparable to the Fast Fourier Transform. In contrast to previous algorithms which proceed either via the Restricted Isometry Property or via filter functions, our approach offers a fresh perspective to the sparse Fourier Transform problem.


==> arxiv/alg.tex <==
In the next lemma, we show the guarantee of $\textsc{LinfinityReduce}$ in Algorithm~\ref{alg:linfinity_reduce}.

\begin{lemma}[guarantee of $\textsc{LinfinityReduce}$ in Algorithm~\ref{alg:linfinity_reduce}]\label{lem:linfinity_reduce}
Let $x \in \C^{[p]^d}$, and $n = p^d$.
Let $R = C_R \log n$, and $B = C_B k$.
Let $C_B \geq 10^6$ and $C_R \geq 10^3$.
Let $\mu = \frac{1}{\sqrt{k}} \|\wh{x}_{-k}\|_2$, and $\nu \geq \mu$.
For $r \in [R]$, let ${\cal T}_r$ be a list of $B$ i.i.d. elements in $[p]^d$.
Let $z \in \C^n$ denote the output of 
\begin{align*}
\textsc{LinfinityReduce} (x, n, y, \{ {\cal T}_r \}_{r=1}^R, \nu).
\end{align*}
Let $S$ be top $C_S k$ coordinates in $\wh{x}$, where $C_S = 26$.
If $\| \wh{x} - y \|_\infty \leq 2 \nu$, $\supp(y) \subseteq S$ and $y$ is independent from the randomness of $\{{\cal T}_r\}_{r=1}^R$, then with probability $1 - 1 / \poly(n)$ under the randomness of $\{ {\cal T}_r \}_{r=1}^R$, $\| \wh{x} - y - z \|_\infty \leq \nu$ and $\supp(z) \subseteq S$.
Moreover, the running time of $\textsc{LinfinityReduce}$ is $O(n \log^2 n)$.
\end{lemma}

\begin{proof}
  
Note that $\forall f \in \ov{S}$, 
\begin{align*}
|\wh{x}_f| \leq \sqrt{ \frac{\|\wh{x}_{-k}\|_2^2} {C_S k - k} } = \frac{1}{5} \mu ,
\end{align*}
where the last step follows from choice of $C_S$.
  
Let $w$ denote the inverse Fourier transform of $y$.
Note that on Line~\ref{lin:u_f_r} in Algorithm~\ref{alg:linfinity_reduce}, for any $f \in [p]^d$ and $r \in [R]$,
\begin{align*}
u_{f,r} = & ~ \frac{\sqrt{n}}{|{\cal T}_r|} \sum_{t \in {\cal T}_r} \omega^{f^\top t} (x_t - w_t) \\
= & ~ \wh{(x-w)}_f^{[{\cal T}_r]} \\
= & ~ \sum_{f'\in [n]} c_{f-f'}^{[{\cal T}_r]} (\wh{x}_{f'}-y_{f'}),
\end{align*}
where the second step follows by the notation in Definition~\ref{def:measurement_notation}, and the third step follows by Lemma~\ref{lem:measurement_decomposition}.
Therefore,
\begin{align}
\wh{x}_f - y_f = & ~ u_{f,r} - \sum_{f' \in [p]^d \setminus \{f\}} c_{f-f'}^{[{\cal T}_r]}(\wh{x}_{f'} - y_{f'}) , \label{eq:noise_decomposition}
\end{align}
By Lemma~\ref{lem:noise_bound},
\begin{align}\label{eq:noise_bound_application}
\Pr_{{\cal T}_r} \left[ \left| \sum_{f' \in [p]^d \setminus \{f\}} c_{f-f'}^{[{\cal T}_r]} (\wh{x}_{f'} - y_{f'}) \right| \geq \frac{10}{\sqrt{B}} \|(\wh{x} - y)_{[p]^d \setminus \{f\}}\|_2 \right] \leq \frac{1}{100}.
\end{align}

We have
\begin{align}\label{eq:bound_hatx_minus_y_bound_nu}
\frac{10}{\sqrt{B}} \|(\wh{x} - y)_{[p]^d \setminus \{f\}}\|_2 \leq & ~ \frac{10}{\sqrt{B}} \left( \| (\wh{x} - y)_{S \setminus \{f\}} \|_2 + \| (\wh{x} - y)_{\ov{S} \setminus \{f\}} \|_2 \right) \notag \\
\leq & ~ \frac{10}{\sqrt{B}} \left( \|\wh{x} - y\|_\infty \cdot \sqrt{|S|} + \|\wh{x}_{\ov{S} \setminus \{f\}}\|_2 \right) \notag \\ 
\leq & ~ \frac{10}{\sqrt{B}} \left( 2 \nu \cdot \sqrt{26 k} + \sqrt{k} \mu \right) \notag \\
\leq & ~ \frac{1}{100\sqrt{k}} \left( 2 \nu \cdot \sqrt{26 k} + \sqrt{k} \mu \right) \notag \\
< & ~ 0.12 \nu,
\end{align}
where the first step following by triangle inequality, the second step follows by the assumption that $\supp(y) \subseteq S$, the forth step follows by $C_B \geq 10^6$, the last step follows by $\mu \leq \nu$. 

Therefore,
\begin{align*}
\Pr_{{\cal T}_r} [|u_{f,r} - (\wh{x}_f-y_f)| \leq 0.12\nu] = & ~ \Pr_{{\cal T}_r} \left[ \left| \sum_{f' \in [p]^d \setminus \{f\}} c_{f-f'}^{[{\cal T}_r]} (\wh{x}_{f'} - y_{f'}) \right| \leq 0.12 \nu \right] \\
= & ~ 1 - \Pr_{{\cal T}_r} \left[ \left| \sum_{f' \in [p]^d \setminus \{f\}} c_{f-f'}^{[{\cal T}_r]} (\wh{x}_{f'} - y_{f'}) \right| > 0.12 \nu \right] \\
\geq & ~ 1 - \Pr_{{\cal T}_r}\left[ \left| \sum_{f' \in [p]^d \setminus \{f\}} c_{f-f'}^{[{\cal T}_r]} (\wh{x}_{f'} - y_{f'}) \right| \geq \frac{10}{\sqrt{B}} \|(\wh{x} - y)_{[p]^d \setminus \{f\}}\|_2 \right] \\
\geq & ~ 1 - \frac{1}{100},
\end{align*}
where the first step follows by \eqref{eq:noise_decomposition}, the third step follows by \eqref{eq:bound_hatx_minus_y_bound_nu}, and the last step follows by \eqref{eq:noise_bound_application}.
 
Thus we have 
\begin{align*}
\Pr_{{\cal T}_r}[ u_{f,r} \in \mathcal{B}_\infty(\wh{x}_f - y_f, 0.12 \nu)] \geq \Pr_{{\cal T}_r} [|u_{f,r} - (\wh{x}_f-y_f)| \leq 0.12\nu] \geq 1 - \frac{1}{100}.
\end{align*}
Let $\eta_f = \text{median}_{r \in [R]} u_{f,r}$ as on Line~\ref{lin:taking_meidan} in Algorithm~\ref{alg:linfinity_reduce}.
By Chernoff bound, with probability $1 - 1/\poly(n)$, more than $\frac{1}{2} R$ elements in $\{u_{f,r}\}_{r=1}^{R}$ are contained in box $\mathcal{B}_\infty(\wh{x}_f - y_f, 0.12 \nu)$, so that $\eta_f \in \mathcal{B}_\infty(\wh{x}_f - y_f, 0.12 \nu)$.

Therefore, we have 
\begin{align*}
\Pr[|\eta_f - (\wh{x}_f - y_f)|  \leq 0.17 \nu] \geq 
\Pr[|\eta_f - (\wh{x}_f - y_f)| \leq \sqrt{2} \cdot 0.12 \nu ] \geq 1 - 1/\poly(n).
\end{align*}
Let $E$ be the event that for all $f \in [p]^d$, $|\eta_f - (\wh{x}_f - y_f)| \leq 0.17 \nu$.
By a union bound over $f \in [p]^d$, event $E$ happens with probability $1 - 1/\poly(n)$.
In the rest of the proof, we condition on event $E$.

({\bf Case 1}) For $f \in \ov{S}$, note that 
\begin{align*}
|\eta_f| \leq 0.17 \nu + |\wh{x}_f - y_f| = 0.17 \nu + |\wh{x}_f| \leq 0.17 \nu + 0.2\nu = 0.37 \nu.
\end{align*}

According to the if statement between Line~\ref{lin:if_eta_begin} and Line~\ref{lin:if_eta_end} in Algorithm~\ref{alg:linfinity_reduce}, $z_f$ will be assigned $0$.
Thus $\supp(z) \subseteq S$.
In addition, $|\wh{x}_f - y_f - z_f| = |\wh{x}_f| \leq \mu \leq \nu$.

({\bf Case 2}) For $f \in S$, we have two cases.
We prove that $|(\wh{x}_f - y_f) - z_f| \leq \nu$ for both cases.

({\bf Case 2.1}) $|\eta_f| < 0.5 \nu$.
$z_f$ is assigned $0$. 
Because 
\begin{align*}
|\eta_f - (\wh{x}_f - y_f)| \leq 0.17 \nu, ~~~ |\wh{x}_f - y_f| \leq |\eta_f| + 0.17 \nu \leq 0.67 \nu.
\end{align*} 
Therefore, 
\begin{align*}
|(\wh{x}_f - y_f) - z_f| \leq 0.67 \nu \leq \nu.
\end{align*}

({\bf Case 2.2}) $|\eta_f| \geq 0.5 \nu$.
$z_f$ is assigned $\eta_f$. We have
\begin{align*}
|(\wh{x}_f - y_f) - z_f| = & ~ |(\wh{x}_f - y_f) - \eta_f| \leq 0.17 \nu \leq \nu.
\end{align*} 

We thus have obtained that with probability $1 - 1/\poly(n)$, $\| (\wh{x} - y) - z \|_\infty \leq \nu$ and $\supp(z) \subseteq S$.

The running time of \textsc{LinfinityReduce} is dominated by the loop between Line~\ref{lin:linfinity_reduce_first_loop_begin} and Line~\ref{lin:linfinity_reduce_first_loop_end}, which takes $O(R \cdot n \log n) = O(n \log^2 n)$ by FFT.
\end{proof}

For a given box $\mathcal{B}_\infty(c, r)$ and grid $\mathcal{G}_{r_g}$, we say a shift $s \in \C$ is good if after applying the shift, all the points in the shifted box $\mathcal{B}_\infty(c, r)+s$ are mapped to the same point by $\Pi_{r_g}$ (recall that $\Pi_{r_g}$ projects any point to the nearst grid point in $\mathcal{G}_{r_g}$). 
We formulate the notion of a good shift in the following definition, and illustrate in Figure~\ref{fig:good_shift}.

\begin{definition}[good shift] \label{def:good_shift}
For any $r_g$, $r_b$, and any $c \in \C$, we say shift $s \in \C$ is a good shift if
\begin{align*}
\left| \Pi_{r_g} ( \mathcal{B}_{\infty} ( c , r_b ) + s ) \right| = 1 .
\end{align*}
\end{definition}

\begin{figure}[!t]
  \centering
    \includegraphics[width=\textwidth]{good_shift}
    \caption{Illustration of good and bad shifts in Definition~\ref{def:good_shift}. 
    In (a), the small square represents box $\mathcal{B}_\infty(c, r_b)$, and the dashed lines represent the decision boundary of $\Pi_{r_g}$.
    The arrows in (b) and (c) represent two different shifts, where the shift in (b) is an example of good shift, since the shifted box does not intersect with the decision boundaries of $\Pi_{r_g}$, while the shift in (c) is an example of bad shift, since the shifted box intersects with the decision boundaries of $\Pi_{r_g}$.
    }\label{fig:good_shift}
\end{figure}

The following lemma intuitively states that if we take a box of radius $r_b$ (or equivalently, side length $2r_b$) and shift it randomly by an offset in $\mathcal{B}_\infty(0, r_s)$ (or equivalently, $[-r_s, r_s] \times [-r_s, r_s]$) where $r_s \geq r_b$, and next we round everyone inside that shifted box to the closest point in $G_{r_g}$ where $r_g \geq 2 r_s$, then with probability at least $(1 - r_b/r_s)^2$ everyone will be rounded to the same point.
In other words, let $s \sim \mathcal{B}_\infty(0, r_s)$, for box $\mathcal{B}_\infty(c, r_b)$ and grid $\mathcal{G}_{r_g}$, $s$ is a good shift with probability at least $(1 - r_b/r_s)^2$.
We illustrate the lemma in Figure~\ref{fig:random_shift_lemma}.

\begin{figure}[!t]
  \centering
    \includegraphics[width=0.8\textwidth]{random_shift_lemma}
    \caption{Illustration of Lemma~\ref{lem:random_shift}. In (a) the smallest square represents box $\mathcal{B}_\infty(c, r_b)$, the medium-sized square represents $\mathcal{B}_\infty(c, r_s)$, and the dashed lines represent decision boundaries of $\Pi_{r_g}$. 
    Note that for $s \sim \mathcal{B}_\infty(0, r_s)$, the center of the shifted box $s + \mathcal{B}_\infty(c, r_b)$ is $s+c \sim \mathcal{B}_\infty(c, r_s)$.
    Shift $s$ is good (recall in Definition~\ref{def:good_shift}) for box $\mathcal{B}_\infty(c, r_b)$ and grid $\mathcal{G}_{r_g}$ if and only if the distance between $s+c$ and decision boundaries of $\Pi_{r_g}$ is greater than $r_b$.
    In (b), we draw in red the set of points which are within distance at most $r_b$ to the decision boundaries of $\Pi_{r_g}$. Then in (b) the red part inside $\mathcal{B}_\infty(c, r_s)$ corresponds to bad shifts (plus $c$), and the green part corresponds to good shifts (plus $c$). 
    Intuitively, the fraction of the green part is at least $(1 - r_b / r_s)^2$ because the vertical red strips can cover a width of at most $2r_b$ on the $x$-axis of $\mathcal{B}_\infty(c, r_s)$ (whose side length is $2r_s$), and the horizontal red strips can cover a width of at most $2r_b$ on the $y$-axis.}\label{fig:random_shift_lemma}
\end{figure}

\begin{lemma}[property of a randomly shifted box]\label{lem:random_shift} 
For any $r_g,r_s,r_b$ so that $r_g/2 \geq r_s \geq r_b > 0$ and any $c \in \C$, let $s \in \C$ be uniform randomly chosen in $\mathcal{B}_\infty(0, r_s)$, then 
\begin{align*}
\Pr_{s \sim \mathcal{B}_\infty(0, r_s)} \Bigg[ \bigg| \Pi_{r_g}( \mathcal{B}_\infty(c, r_b) +s) \bigg| = 1 \Bigg] \geq \left( 1 - \frac{r_b}{r_s} \right)^2,
\end{align*}
where we refer $r_g,r_s,r_b$ as the radius of grid, shift and box respectively, and we use notation $C + s$ to refer to $\{c+s: c \in C\}$.
\end{lemma}

\begin{proof}
We consider complex numbers as points in $2$D plane, where the real part is the coordinate on $x$-axis, and the imaginary part is the coordinate on $y$-axis.
Note that the ``decision boundary'' of projection $\Pi_{r_g}$ from $\C$ onto grid $\mathcal{G}_{r_g}$ consists of vertical lines of form $x = (m + \frac{1}{2}) r_g$ and horizontal lines of form $y = (m + \frac{1}{2}) r_g$, where $m \in \Z$.
$\left| \Pi_{r_g}( \mathcal{B}_\infty(c, r_b) +s) \right| = 1$ if and only if the shifted box $\mathcal{B}_\infty(c, r_b) +s$ does not intersect with the ``decision boundary''.

Let $s = s_x + s_y \i$ and $c = c_x + c_y \i$. 
Then the shifted box does not intersect with the ``decision boundary'' if and only if both intervals 
\begin{align*}
[c_x - r_b + s_x, c_x + r_b + s_x] \text{~and~} [c_y - r_b + s_y, c_y + r_b + s_y]
\end{align*}
do not intersect with $\{(m+\frac{1}{2})r_g: m \in \Z \}$.
The probability of each one is at least $1 - \frac{r_b}{r_s}$, and two events are independent.
Therefore, we get the claimed result.
\end{proof}

In the following, we define event $\mathcal{E}$, which is a sufficient condition for the correctness of Algorithm~\ref{alg:fourier_sparse_recovery}.
Event $\mathcal{E}$ consists of three parts. 
Part~1 of $\mathcal{E}$ is used to prove that $a_\ell \leq 10 
\log n$ for $\ell \in [L-1]$ on Line~\ref{lin:a_ell} in Algorithm~\ref{alg:fourier_sparse_recovery}.
Part~2 and Part~3 of $\mathcal{E}$ are used to prove that Line~\ref{lin:nu_ell} to Line~\ref{lin:z_assign} in Algorithm~\ref{alg:fourier_sparse_recovery} give a desirable $z^{(\ell)}$ for $\ell \in [L]$.

\begin{definition}[sufficient condition for the correctness of Algorithm~\ref{alg:fourier_sparse_recovery}] \label{def:sufficient_event}
For input signal $x \in \C^n$, let $\mu = \frac{1}{\sqrt{k}} \|\wh{x}_{-k}\|_2$ and $R^*$ is an upper bound of $\|\wh{x}\|_\infty / \mu$.
Let $S$ be top $C_S k$ coordinates in $\wh{x}$.
Let $H = \min \{ \log k + C_H, \log R^* \}$, and $L = \log R^* - H + 1$.
For $\ell \in [L]$, let $\nu_\ell = 2^{-\ell} \mu R^*$.
For $\ell \in [L-1]$, let $s_\ell^{(a)}$ be the $a$-th uniform randomly sampled from $\mathcal{B}_\infty(0, \alpha \nu_\ell)$ as appeared on Line~\ref{lin:shift} in Algorithm~\ref{alg:fourier_sparse_recovery} (i.e. $s_\ell^{(1)}, \ldots, s_\ell^{(a_\ell)}$ are sampled, and $s_\ell^{(a_\ell)}$ is the first that satisfies the condition on Line~\ref{lin:until_good}).
For the sake of analysis, we assume that Algorithm~\ref{alg:fourier_sparse_recovery} actually produces an infinite sequence of shifts $s_\ell^{(1)}, s_\ell^{(2)}, \ldots$, and chooses the smallest $a_\ell$ so that $s_\ell^{(a_\ell)}$ satisfies $\forall f \in \supp(y^{(\ell-1)}+z^{(\ell)}), |\Pi_{\beta \nu_\ell}(\mathcal{B}_\infty(y^{(\ell-1)}_f + z^{(\ell)}_f + s_\ell^{(a_\ell)}, 2^{1-H} \nu_\ell))|=1$ on Line~\ref{lin:until_good}.

For $\ell \in [L-1]$, we define random variable $a'_\ell$ to be the smallest $a'$ such that for all $f \in S$,
 \begin{align*}
 \left| \Pi_{\beta \nu_\ell} \left(\mathcal{B}_\infty(\wh{x}_f + s_\ell^{(a')}, 2^{3-H} \nu_\ell) \right) \right| = 1.
 \end{align*}

We define event $\mathcal{E}$ to be all of the following events hold. \\
1. For all $\ell \in [L-1]$, $a'_\ell \leq 10 \log n$. \\
2. For $\ell = 1$, if we execute Line~\ref{lin:nu_ell} to Line~\ref{lin:z_assign} in Algorithm~\ref{alg:fourier_sparse_recovery} with $y^{(0)} = 0$, we get $z^{(1)}$ such that $\|\wh{x} - z^{(1)}\|_\infty \leq 2^{1-H} \nu_1$ and $\supp(z^{(1)}) \subseteq S$. \\
3. For all $\ell \in \{2, \ldots, L\}$, for all $a \in [10 \log n]$, if we execute Line~\ref{lin:nu_ell} to Line~\ref{lin:z_assign} in Algorithm~\ref{alg:fourier_sparse_recovery} with $y^{(\ell-1)} = \xi$ where
\begin{align*}
\xi_f = 
\begin{cases} 
  \Pi_{\beta \nu_\ell}(\wh{x}_f + s_{\ell-1}^{(a)}), & \text{~if~} f \in S; \\ 
  0, & \text{~if~} f \in \ov{S}.
\end{cases} 
\end{align*}
then we get $z^{(\ell)}$ such that $\|\wh{x} - y^{(\ell-1)} - z^{(\ell)}\|_\infty \leq 2^{1-H} \nu_\ell$  and $\supp(y^{(\ell-1)}+z^{(\ell)}) \subseteq S$.

\end{definition}

In the following, we will prove that for fixed $x$, under the randomness of $\{s_\ell^{(a)}\}_{\ell \in[L-1], a\in\{1,\ldots\}}$ and $\mathcal{T} = \{\mathcal{T}^{(h)}\}_{h\in[H]}$, event $\mathcal{E}$ (defined in Definition~\ref{def:sufficient_event}) happens with probability at least $1 - 1 / \poly(n)$.
Moreover, we will prove that event $\mathcal{E}$ is a sufficient condition for the correctness of Algorithm~\ref{alg:fourier_sparse_recovery}.
Namely, conditioned on event $\mathcal{E}$, Algorithm~\ref{alg:fourier_sparse_recovery} gives a desirable output. 

\begin{lemma}[event $\mathcal{E}$ happens with high probability]\label{lem:E_happen_whp}
Let $\mathcal{E}$ in Definition~\ref{def:sufficient_event}. For any fixed $x \in \C^n$, under the randomness of shifts $\{s_\ell^{(a)}\}_{\ell \in [L-1], a \in \{1,\ldots\}}$ and $\mathcal{T} = \{ \mathcal{T}^{(h)}\}_{h \in [H]}$, 
\begin{align*}
\Pr[\mathcal{E}] \geq 1 - 1/\poly(n).
\end{align*}
\end{lemma}

\begin{proof}
We bound the failure probability of each parts in event $\mathcal{E}$ respectively as follows, and $\Pr[\mathcal{E}] \geq 1 - 1/\poly(n)$ follows by a union bound.


{\bf Part 1.} If $H = \log R^*$, then $L = 1$ and it is trivially true that ``for all $\ell \in [L-1], a'_\ell \leq 10 \log n$''. Otherwise, we have $H = \log k + C_H$. By Lemma~\ref{lem:random_shift}, for any $\ell \in [L-1]$, for any $f \in S$,
\begin{align*}
\Pr_{s \sim \mathcal{B}_\infty(0, \alpha \nu_\ell)} \Bigg[ \bigg| \Pi_{\beta \nu_\ell} \left( \mathcal{B}_\infty \left( \wh{x}_f, 2^{3-H}\nu_\ell \right) +s \right) \bigg| = 1 \Bigg] \geq \left( 1 - \frac{2^{3-H}\nu_\ell}{\alpha \nu_\ell} \right)^2 = \left( 1 - \frac{2^{3-H}}{\alpha} \right)^2 ,
\end{align*}
where $(1 - 2^{3-H} / \alpha)^2 \geq 1 - 2^{4- C_H - \log k} / \alpha \geq 1 - \frac{1}{100 k}$ by our choice of $\alpha$ and $C_H$ in Table~\ref{tab:parameters}.

For each $\ell \in [L-1]$, by a union bound over all $f$ in $S$, the probability is at least $ 1 - \frac{C_S k}{100k} = 1 - \frac{26k}{100k} \geq \frac{1}{2}$ that for all $f \in S$, $|\Pi_{\beta \nu_\ell}(\mathcal{B}_\infty(\wh{x}_f + s, 2^{3-H} \nu_\ell))| = 1$ where $s \sim \mathcal{B}_\infty(0, \alpha \nu_\ell)$. Formally, we get
\begin{align*}
\Pr_{s \sim \mathcal{B}_\infty(0, \alpha \nu_\ell)} \Bigg[  \bigg| \Pi_{\beta \nu_\ell} \left( \mathcal{B}_\infty \left( \wh{x}_f, 2^{3-H}\nu_\ell \right) +s \right) \bigg| = 1, \forall f \in S \Bigg] \geq 1/2.
\end{align*}


Therefore, by definition of $a'_\ell$ in Definition~\ref{def:sufficient_event},
\begin{align*}
\Pr[a'_\ell \leq 10\log n] \geq 1 - (1 / 2)^{10 \log n} = 1 - 1 / n^{10}.
\end{align*}
By a union bound over all $\ell \in [L-1]$, the probability is at least $1 - L / n^{10} = 1 - 1 / \poly(n)$ that for all $\ell \in [L-1]$, $a'_\ell \leq 10 \log n$.


{\bf Part 2.} By Lemma~\ref{lem:linfinity_reduce} and a union bound over all $h \in [H]$, the failure probability is at most $H / \poly(n) = 1 / \poly(n)$, where $H = O(\log k)$ and so $H / \poly(n)$ is still $1 / \poly(n)$.


{\bf Part 3.} For each $\ell \in \{2, \ldots, L\}$ and $a \in [10 \log n]$, similar to the above argument, each has failure probability at most $1 / \poly(n)$.
By a union bound, the failure probability is at most 
\begin{align*}
(L - 1) \cdot (10 \log n) / \poly(n) = 1 / \poly(n).
\end{align*}

\end{proof}

In the following lemma, we show that if event $\mathcal{E}$ (defined in Definition~\ref{def:sufficient_event}) happens, then Algorithm~\ref{alg:fourier_sparse_recovery} gives a desirable output.

\begin{lemma}[correctness of Algorithm~\ref{alg:fourier_sparse_recovery} conditioned on $\mathcal{E}$]\label{lem:correctness_of_fourier_sparse_recovery}
Let $n = p^d$, and let $k \in [n]$.
Let $x \in \C^{n}$ be input signal.
Let $\mu = \frac{1}{\sqrt{k}} \|\wh{x}_{-k}\|_2$. 
Let $R^* \geq \|\wh{x}\|_\infty\ / \mu$ and $R^*$ is a power of $2$. 
Let $H = \min \{\log k + C_H, \log R^*\}$.
Let $L = \log R^* - H + 1$.
For $\ell \in [L-1]$, let $y^{(\ell)}$ be the vector obtained on Line~\ref{lin:y_ell_assign} of Algorithm~\ref{alg:fourier_sparse_recovery}.
For $\ell \in [L]$, let $z^{(\ell)}$ be the vector obtained on Line~\ref{lin:z_assign}.
Note that $y^{(0)} = 0$, and $y^{(L-1)}+z^{(L)}$ is the output of $\textsc{FourierSparseRecovery}(x,n,k,R^*,\mu)$ in Algorithm~\ref{alg:fourier_sparse_recovery}.
Conditioned on the event $\mathcal{E}$ (defined in Definition~\ref{def:sufficient_event}) happens, we have 
\begin{align*}
\| \wh{x} - y^{(L-1)} - z^{(L)} \|_\infty \leq \frac{1}{\sqrt{k}} \|\wh{x}_{-k}\|_2.
\end{align*}
\end{lemma}

\begin{proof}
We first discuss the case that $H = \log R^*$.
In that case, $L = 1$. 
Conditioned on the event $\mathcal{E}$ (Part~2 of $\mathcal{E}$), $z^{(1)}$ obtained through Line~\ref{lin:nu_ell} to Line~\ref{lin:z_assign} in Algorithm~\ref{alg:fourier_sparse_recovery} satisfies $\|\wh{x} - z^{(1)}\|_\infty \leq 2^{1-H} \nu_1 = 2^{1-H} (2^{-1}\mu R^*) = \mu$.

In the rest of the proof, we discuss the case that $H > \log R^*$.
For $\ell \in [L]$, let $\nu_\ell = 2^{-\ell} \mu R^*$.
For $\ell \in [L-1]$, let $s_\ell^{(a_\ell)} \in \mathcal{B}_\infty(0, \alpha \nu_\ell)$ denote the first $s_\ell^{(a)}$ on Line~\ref{lin:shift} in Algorithm~\ref{alg:fourier_sparse_recovery} such that for all $f \in \supp(y^{(\ell-1)}+z^{(\ell)})$,
\begin{align*}
\left| \Pi_{\beta \nu_\ell} \left( \mathcal{B}_\infty \left( y_f^{(\ell-1)} + z^{(\ell)}_f + s_\ell^{(a)}, 2^{1-H} \nu_\ell \right) \right) \right|=1.
\end{align*}
For $\ell \in [L-1]$, we define $\xi^{(\ell)} \in \C^{[p]^d}$ as follows
\begin{align*}
\xi_f^{(\ell)} = 
\begin{cases} 
  \Pi_{\beta \nu_\ell}(\wh{x}_f + s_\ell^{(a_\ell)}), & \text{~if~} f \in S; \\ 
  0, & \text{~if~} f \in \ov{S}.
\end{cases}
\end{align*}
We also define $\xi^{(0)} = 0$, $s_0^{(a)} = 0$ for $a \in \{1,\ldots\}$ and $a_0 = 1$.

({\bf Goal: Inductive Hypothesis}) We are going to prove that conditioned on event $\mathcal{E}$ (defined in Definition~\ref{def:sufficient_event}), for all $\ell \in \{0,\ldots, L-1\}$, 
\begin{align*}
y^{(\ell)} = \xi^{(\ell)} \text{~~~and~~~} a_\ell \leq 10 \log n.
\end{align*}

({\bf Base case}) Note that $y^{(0)} = \xi^{(0)} = 0$ and $a_0 = 1 \leq 10 \log n$. 

({\bf Inductive step}) We will prove that conditioned on event $\mathcal{E}$, if $y^{(\ell-1)} = \xi^{(\ell-1)}$ and $a_{\ell-1} \leq 10 \log n$ for $\ell \in [L-1]$, then $y^{(\ell)} = \xi^{(\ell)}$ and $a_\ell \leq 10 \log n$.

({\bf Proving $a_\ell \leq 10 \log n$}) Conditioned on event $\mathcal{E}$ (if $L=1$ then from Part~2 of $\mathcal{E}$, otherwise from Part~3 of $\mathcal{E}$ and by the fact that $a_{\ell-1} \leq 10 \log n$), $z^{(\ell)}$ obtained through Line~\ref{lin:nu_ell} to Line~\ref{lin:z_assign} in Algorithm~\ref{alg:fourier_sparse_recovery} satisfies $\|\wh{x} - \xi^{(\ell-1)} - z^{(\ell)}\|_\infty \leq 2^{1-H} \nu_\ell$ and $\supp(z^{(\ell)}) \subseteq S$.
Namely, for all $f \in [p]^d$, $\xi_f^{(\ell-1)} + z^{(\ell)}_f \in \mathcal{B}_\infty(\wh{x}_f, 2^{1-H} \nu_\ell)$.
Recall the definition of $a_\ell'$ in Definition~\ref{def:sufficient_event}.
We can prove that $a_\ell \leq a_\ell'$ because if for all $f \in S$, 
\begin{align*}
\left| \Pi_{\beta \nu_\ell} \left(\mathcal{B}_\infty \left( \wh{x}_f + s_\ell^{(a'_\ell)}, 2^{3-H} \nu_\ell \right) \right) \right| = 1,
\end{align*}
then for all $f \in \supp(y^{(\ell-1)}+z^{(\ell)})$, 
\begin{align*}
\left| \Pi_{\beta \nu_\ell} \left( \mathcal{B}_\infty \left( y^{(\ell-1)}_f + z^{(\ell)}_f + s_\ell^{(a'_\ell)}, 2^{1-H} \nu_\ell \right) \right) \right|=1
\end{align*}
where 
\begin{align*}
\mathcal{B}_\infty \left( y^{(\ell-1)}_f + z^{(\ell)}_f + s_\ell^{(a'_\ell)}, 2^{1-H} \nu_\ell \right) \subseteq \mathcal{B}_\infty \left( \wh{x}_f + s_\ell^{(a'_\ell)}, 2^{3-H} \nu_\ell \right)
\end{align*}
which follows by $\xi_f^{(\ell-1)} + z^{(\ell)}_f \in \mathcal{B}_\infty(\wh{x}_f, 2^{1-H} \nu_\ell)$.
Therefore, conditioned on $\mathcal{E}$ (Part~1 of $\mathcal{E}$), $a_\ell \leq a_\ell' \leq 10 \log n$. 


({\bf Proving $y^{(\ell)}_f = \xi^{(\ell)}_f$}) For $f \in [p]^d$, we will prove that $y^{(\ell)}_f = \xi^{(\ell)}_f$ in two cases.

({\bf Case 1}) If $f \in \supp(y^{(\ell-1)} + z^{(\ell)}) \subseteq S$. We have 
\begin{align*}
y_f^{(\ell)} 
= & ~ \Pi_{\beta \nu_\ell} \left( y^{(\ell-1)}_f + z^{(\ell)}_f + s_\ell^{(a_\ell)} \right) \\
= & ~ \Pi_{\beta \nu_\ell} \left( \xi^{(\ell-1)}_f + z^{(\ell)}_f + s_\ell^{(a_\ell)} \right).
\end{align*} 
Because $\xi_f^{(\ell-1)} + z^{(\ell)}_f \in \mathcal{B}_\infty(\wh{x}_f, 2^{1-H} \nu_\ell)$, we have $\xi^{(\ell-1)}_f + z^{(\ell)}_f + s_\ell^{(a_\ell)} \in \mathcal{B}_\infty(\wh{x}_f + s_\ell^{(a_\ell)}, 2^{1-H} \nu_\ell)$.
By the choice of $s_\ell^{(a_\ell)}$, $\Pi_{\beta \nu_\ell}(\xi^{(\ell-1)}_f + z^{(\ell)}_f + s_\ell^{(a_\ell)}) = \Pi_{\beta\nu_\ell}(\wh{x}_f + s_\ell^{(a_\ell)})$.
Thus $y_f^{(\ell)} = \xi_f^{(\ell)}$.

({\bf Case 2}) If $f \not\in \supp(y^{(\ell-1)} + z^{(\ell)})$. We have $y_f^{(\ell)} = 0$.
Because $\xi_f^{(\ell-1)} + z^{(\ell)}_f \in \mathcal{B}_\infty(\wh{x}_f, 2^{1-H} \nu_\ell)$, we have $|\wh{x}_f| < 2^{2 - H} \nu_\ell < 0.1 \beta \nu_\ell$ by our choice of $H$.
We can easily prove that $\xi_f^{(\ell)} = 0 = y_f^{(\ell)}$ in the following two cases: 

({\bf Case 2.1}) If $f \in S$, we have $\xi_f^{(\ell)} = \Pi_{\beta \nu_\ell}(\wh{x}_f + s_\ell^{(a_\ell)}) = 0$ because
\begin{align*}
|\wh{x}_f| + |s_\ell^{(a_\ell)}| < 0.1 \beta \nu_\ell + 2 \alpha \nu_\ell < 0.5 \beta \nu_\ell.
\end{align*}

({\bf Case 2.2}) If $f \in \ov{S}$,  $\xi_f^{(\ell)} = 0$ by definition of $\xi^{(\ell)}$.

Therefore, for all $\ell \in [L-1]$, $y^{(\ell)} = \xi^{(\ell)}$ and $a_\ell \leq 10 \log n$.
Again conditioned on event $\mathcal{E}$ (Part~3 of $\mathcal{E}$), $z^{(L)}$ obtained through Line~\ref{lin:nu_ell} to Line~\ref{lin:z_assign} in Algorithm~\ref{alg:fourier_sparse_recovery} satisfies 
\begin{align*}
\|\wh{x} - y^{(L-1)} - z^{(L)}\|_\infty \leq 2^{1-H} \nu_L = 2^{1-H} (2^{-(\log R^* - H +1)}\mu R^*) = \mu.
\end{align*}
Therefore, $y^{(L-1)} + z^{(L)}$ on Line~\ref{lin:return_recovered_signal} gives a desirable output.

\end{proof}

Now we present our main theorem, which proves the correctness of Algorithm~\ref{alg:fourier_sparse_recovery}, and shows its sample complexity and time complexity.

\begin{theorem}[main result, formal version]\label{thm:fourier_sparse_recovery_formal}
Let $n = p^d$ where both $p$ and $d$ are positive integers.
Let $x \in \C^{[p]^d}$.
Let $k \in \{1, \ldots, n\}$. 
Assume we know $\mu = \frac{1}{k} \|\wh{x}_{-k}\|_2$ and $R^* \geq \|\wh{x}\|_\infty / \mu$ where $\log R^* = O(\log n)$.
There is an algorithm (Algorithm~\ref{alg:fourier_sparse_recovery}) that takes $O(k \log k \log n)$ samples from $x$, runs in $O(n \log^3 n \log k)$ time, and outputs a $O(k)$-sparse vector $y$ such that
\begin{align*}
\| \wh{x} - y \|_{\infty} \leq \frac{1}{\sqrt{k}}\min_{k-\sparse~x'} \| \wh{x} - x' \|_2
\end{align*}
holds with probability at least $1 - 1 / \poly(n)$.
\end{theorem}

\begin{proof}
The correctness of Algorithm~\ref{alg:fourier_sparse_recovery} follows directly from Lemma~\ref{lem:E_happen_whp} and Lemma~\ref{lem:correctness_of_fourier_sparse_recovery}.
The number of samples from $x$ is 
\begin{align*}
B \cdot R \cdot H = O(k \cdot \log n \cdot \log k) = O(k \log k \log n).
\end{align*}
Its running time is dominated by $L \cdot H = O(\log k \log n)$ invocations of \textsc{LinfinityReduce} (in Algorithm~\ref{alg:linfinity_reduce}).
By Lemma~\ref{lem:linfinity_reduce}, the running time of \textsc{LinfinityReduce} is $O(n \log^2 n)$.
Therefore, the running time of Algorithm~\ref{alg:fourier_sparse_recovery} is 
\begin{align*}
O(L \cdot H \cdot n \log^2 n) = O( \log k \cdot \log n \cdot n \log^2 n ) = O( n \log^3 n \log k).
\end{align*}
\end{proof}

%\textsc{LinfReduce}
%\textsc{LinfinityReduce}


==> arxiv/dis.tex <==
\newpage
\section{Some Not So Useful Discussions}
\Zhao{This section probably has nothing to do with our main result for optimal sample $d$-dimensional Fourier transform. We can ignore it for now, and remove it later.}

We will assume that $x(t) = x^*(t) + g(t)$, and $x^*(t)$ has a $k$-sparse Fourier representation.

We will need the following lemma.

\begin{lemma} \label{lem:primes}
Pick $ R = c \log k $ primes in $[ C k \log (FT), 2C k \log (FT) ]$. Let this set be $P$. Then, for any $S \subseteq \{ -FT, \ldots -1, 0, 1 , \ldots , FT\}$ of $k$ elements, we have that the following holds with $1- 1/k$ probability.

For every $x \in S$ there exist at least $2R/3$ primes in $P$ such that $x \neq y \pmod p$ for every $ y \in S \setminus \{x\}$.
\end{lemma}

\begin{proof}(Sketch)
By the prime number theorem, there exist $\beta k \log (FT) / (\log k + \log\log FT)$ primes in that interval, where $\beta$ is at least $\frac{C}{\log C}$. 
% \Zhengyu{to be more exact, there are $\Theta( k \log (FT) / (\log k + \log\log FT))$ primes. If $\log\log FT = \omega(\log k)$, then the number of primes is not what you wrote.}
For all $x,y \in \{ -FT, \ldots -1, 0, 1 , \ldots , FT\}$, we have that $x - y$ can have at most $\alpha \log (FT) / (\log k + \log\log FT)$ prime factors in that interval, for some constant $\alpha$.

Thus, for fixed $x,y$ the probability that a random prime in $[ C k \log (FT), 2C k \log (FT) ]$ divides $x-y$ is upper bounded by 
\begin{align*}
\frac{\alpha \log (FT) / (\log k + \log\log FT)}{\beta k \log (FT) / (\log k + \log\log FT)} = \frac{\alpha}{\beta} \frac{1}{k} \leq \frac{1}{10k},
\end{align*}
where the last step follows from $\beta \geq \frac{C}{\log C}$ and $C$ is sufficiently large.
Thus, for fixed $x \in S$, with constant probability a random prime will not divide anyone in the set $\{ x-y: y \in S \setminus \{x\} \}$. 
By Chernoff bound, if we are taking $R = c \log k$ random primes for large enough $c$, then with probability $1 - 1/\poly(k)$, at least $\frac{2}{3} R$ of them will not divide any element in the set $\{ x-y: y \in S \setminus \{x\} \}$.
A union bound on all $x \in S$ concludes the lemma.  
% \Zhao{I don't understand the meaning of $ x - ( S \setminus \{ x \} )$}
\end{proof}


We will also need the next Lemma.

\begin{lemma} \label{lem:alias}
Let $y$ be a signal with $k$-sparse Fourier representation
\begin{align*}
	y(t) = \sum_{ j= 1}^k v_j e^{2\pi \iu f_j t }.
\end{align*}
Let $\wh{z}$ denote the $p$-dimensional Fourier transform of the vector
$z$ with $z_j = y(j / ( \eta p) )$. Then, % \Zhao{$z_j = y_{ j / (\eta p) }$ ?} %the result is a vector the $i$th coordinate of which equals
\begin{align*}
\wh{z}_i = \sum_{ j : (f_j/\eta) = i \pmod p} v_j.
\end{align*}
\end{lemma}

\begin{proof}
\begin{align*}
\wh{z}_i = & ~ \frac{1}{p} \sum_{s = 1} ^ {p} e^{-2 \pi \iu s i /p} z_s \\
= & ~ \frac{1}{p} \sum_{s = 1} ^ {p} e^{-2 \pi \iu s i /p} y(s/(\eta p)) \\
= & ~ \frac{1}{p} \sum_{s = 1} ^ {p} e^{-2 \pi \iu s i /p} \sum_{j = 1} ^ {k} v_j e^{2 \pi \iu f_j s / (\eta p)} \\
= & ~ \frac{1}{p} \sum_{j = 1} ^ {k} v_j \sum_{s = 1} ^ {p} e^{2 \pi \iu f_j s / (\eta p) - 2 \pi \iu s i /p} \\
= & ~ \frac{1}{p} \sum_{j = 1} ^ {k} v_j \sum_{s = 1} ^ {p} e^{2 \pi \iu \frac{s}{p} (\frac{f_j}{\eta} - i)} \\
\end{align*}
\Zhengyu{If $\frac{f_j}{\eta}$ is an integer, then $\sum_{s = 1} ^ {p} e^{2 \pi \iu \frac{s}{p} (\frac{f_j}{\eta} - i)} = 1_{(f_j/\eta) = i \pmod p}$. But what if $\frac{f_j}{\eta}$ is not an integer?}
\Vasileios{ Let us fix firs t the case that $f_j$ are multiples of $C \eta$, for some constant $C$}
\end{proof}


Now, which is the idea? Take the $R$ random primes, and consider signal $x$ with Lemma~\ref{lem:alias} and all these random primes. For most primes the $v_j$ will be isolated, hence you can read them. Call these samples Set $1$. Consider also $y(t - 1)$, which has Fourier transform by the shift Theorem,
\begin{align*}
y(t - 1) = \sum_{j=1}^k \left(v_j e^{-2\pi f_j} \right) \cdot e^{2 \pi f_j t }. 
\end{align*}

Using Lemma \ref{lem:alias} and the above observation, as well as the samples from Set $1$, we can infer the $f_j$.

\begin{lemma} \label{lem:alias_2}
Consider signal $x'(t) = x^*(t+1)$. Let $\hat{w}$ denote the $p$-dimensional Fourier transform of the vector $w$ with $w_j = x'(j/(\eta p))$. Then,
\begin{align*}
	\hat{w}_i = \sum_{ j : (f_j/\eta) = i \pmod p} e^{2 \i \pi f_j} v_j.	
\end{align*}
%\Zhao{What is $w'$? I don't understand the summation. I don't understand $e^{2\pi f_j} v_j$ also, should it be $e^{2\pi \i f_j t} v_j$ or $e^{2\pi \i f_j}$?}
\end{lemma}

Using Lemma \ref{lem:alias} and \ref{lem:alias_2} with the primes from Lemma \ref{lem:primes}  we can find $v_j$ and $f_j$ in $O( k \log (FT) \log k)$ sample and time. The duration is $O(1/\eta)$, and we can perfectly reconstruct the signal if $g = 0$.

\begin{comment}
\begin{algorithm}
\begin{algorithmic}
\Procedure{aa}{}
	\State
\EndProcedure
\end{algorithmic}
\end{algorithm}
\end{comment}


==> arxiv/intro.tex <==
\section{Introduction}

Initiated in discrete signal processing, compressed sensing/sparse recovery is an extensively studied branch of mathematics and algorithms, which postulates that a small number of linear measurements suffice to approximately reconstruct the best $k$-sparse approximation of a vector $x\in \mathbb{C}^n$ \cite{ct06,crt06,d06}. 
Besides substantial literature on the subject, compressed sensing has wide real-world applications in imaging, astronomy, seismology, etc. 
One of the initial papers in the field, Candes, Romberg and Tao \cite{crt06a}, has almost $15,000$ references.

Probably the most important subtopic is sparse Fourier transform, which aims to reconstruct a $k$-sparse vector from Fourier measurements. 
In other words, measurements are confined to the so-called Fourier ensemble. In Optics imaging \cite{g05,v11} and Magnetic resonance imaging (\textsc{MRI}) \cite{assn08}, the physics \cite{r89} of the underlying device restricts us to the Fourier ensemble, where the sparse Fourier problem becomes highly relevant. In fact, these applications became one of the inspirations for Candes, Romberg and Tao. 
The number of samples plays a crucial role: they determine the amount of radiation a patient receives in CT scans and taking fewer samples can reduce the amount of time the patient needs to spend in the machine. %, since they can allow speeding up the process of imaging. \Zhengyu{I think taking fewer measurements atomically reduce the amount of time a patient stays in the machine}
The framework has found its way in life-changing applications, including \textsc{Compressed Sensing GRAB-VIBE}, \textsc{CS SPACE}, \textsc{CS SEMAC} and \textsc{CS TOF} by Siemens \cite{siemens}, and Compressed Sense by Phillips \cite{phillips}. 
Its incorporation into the MRI technology allows faster acquisition rates, depiction of dynamic processes or moving organs, as well as acceleration of \textsc{MRI} scanning up to a factor of $40$. 
In the words of \textsc{SIEMENS} Healthineers: 

{ \emph{ This allows bringing the advantages of Compressed Sensing \textsc{GRASP-VIBE} to daily clinical routine.
\begin{itemize}
\item Perform push-button, free-breathing liver dynamics.
\item Overcome timing challenges in dynamic imaging and respiratory artifacts.
\item Expand the patient population eligible for abdominal \textsc{MRI}.
\end{itemize}
}}

On the other hand, Fourier transform is ubiquitous: image processing, audio processing, telecommunications, seismology, polynomial multiplication, \textsc{Subset Sum} and other textbook algorithms are some of the best-known applications of Fast Fourier Transform. 
The Fast Fourier Transform (FFT) by Cooley and Tukey \cite{ct65} runs in $O(n \log n)$ time and has far-reaching impact on all of the aforementioned cases. We can thus expect that algorithms which exploit sparsity assumptions about the input and can outperform FFT in applications are of high practical value. 
Generally, the two most important parameters one would like to optimize are sample complexity, i.e. the numbers needed to obtain from the time domain, as well as the time needed to approximate the Fourier Transform. 


Two different lines of research exist for the problem: one focuses solely on sample complexity, while the other tries to achieve sublinear time while keeping the sample complexity as low as possible. 
The first line of research operates via the renowned Restricted Isometry Property (RIP), which proceeds by taking random samples and solving a linear/convex program, or an iterative thresholding procedure \cite{ct06,ddts06,tg07,bd08,dm08,rv08,bd09short,bd09,nt09,nv09,gk09,bd10,nv10,f11,b14,hr16}. Such algorithms are analyzed in two steps as follows: 
The first step ensures that, after sampling an appropriate number of points from the time domain, the inverse DFT matrix restricted on the rows indexed by those points acts as a near isometry on the space of $k$-sparse vectors. 
All of the state-of-the-art results \cite{ct06,rv08,b14,hr16} employ chaining arguments to make the analysis of this sampling procedure as tight as possible. 
The second part is to exploit the aforementioned near-isometry property to find the best $k$-sparse approximation to the signal. 
There, existing approaches either follow an iterative procedure which gradually denoise the signal \cite{bd08,nt09,nv09}, or perform $\ell_1$ minimization \cite{ct06}, a method that promotes sparsity of solutions.

The second line of research tries to implement arbitrary linear measurements via sampling Fourier coefficients \cite{gl89,m92,km93,ggims02,ags03,gms05,i08,i10,hikp12a,hikp12b,lawlor13,iw13,PR14,ikp14,ik14,k16,k17,ci17,bzi17,mzic2017,ln19} and use sparse functions (in the time domain) which behave like bandpass filters in the frequency domain. 
The seminal work of Kapralov \cite{k17} achieves $O(k \log n)$ samples and running time that is some $\log $ factors away from the sample complexity. 
This would be the end of the story, if not for the fact that this algorithm does not scale well with dimension, since it has an exponential dependence on $d$. 
Indeed, in many applications, one is interested in higher dimensions, rather than the one-dimensional case. 
The main reason\footnote{But not the only one: pseudorandom permutations for sparse FT in high dimensions also incur an exponential loss, and it is not known whether this can be avoided.} why this curse of dimensionality appears is the lack of dimension-independent ways to construct functions that approximate the $\ell_\infty$ ball and are sufficiently sparse in the time domain. 
A very nice work of Kapralov, Velingker and Zandieh \cite{kvz19} tries to remedy that by combining the standard execution of FFT with careful aliasing, but their algorithm works in a noiseless setting, and has a polynomial, rather than linear, dependence on $k$; the running time is polynomial in $k, \log n$ and the exponential dependence is avoided. 
It is an important and challenging question whether a robust and more efficient algorithm can be found. 

We note that in many applications, such as MRI or computed tomography (CT), the main focus is the sample complexity; the algorithms that have found their way to industry are, to the best of our knowledge, not concerned with sublinear running time, but with the number of measurements, which determine the acquisition time, or in CT the radiation dose the patient receives. 
Additionally, it is worth noting some recent works on sparse Fourier transform in the continuous setting, see \cite{i10,iw13,iw13,bcgls14,ps15,ckps16,s17,hkmmvz19,cp19a,cp19b,song19}.

\paragraph{Our Contribution.} We give a new algorithm for the sparse Fourier transform problem, which has $O( k \log n \log k)$ sample complexity for any dimension, and achieves the $\ell_\infty/\ell_2$ guarantee\footnote{This is the strongest guarantee in the sparse recovery literature. See also the caption of the table in Section 1.2}, while running in time $\tilde{O}(n)$. 
The previous state-of-the-art algorithm that achieved such a guarantee is the work of Indyk and Kapralov \cite{ik14}, which has $ 2^{O(d \log d)} k \log n $ sample complexity; an exponentially worse dependence on $d$. 
The work of \cite{hr16} obtains $O(k \log n \log^2k)$ samples in any dimension, but has a much weaker error guarantee\footnote{They achieve $\ell_2/\ell_1$ instead of $\ell_\infty/\ell_2$, see next Section for comparison. }, while their approach requires $\Omega( k \log n \log k)$ samples in high dimensions \cite{r19}. 
Moreover, the algorithm in \cite{ik14} operates when the universe size in each dimension is a power of $2$, whereas there is no restriction in our work. 
To obtain our result, we introduce a set of new techniques, deviating from previous work, which used the Restricted Isometry Property and/or filter functions. 

%\Zhao{I feel the above section should be moved into Our result section. Currently our result only sells $\ell_{\infty}/\ell_2$, it is very strange to me..}

%In \cite{hikp12a}, it explicitly mentioned that ``Extend the algorithm to the case when $n$ is not a power of $2$'' is an open question \Vasileios{ I do not think we should put it here. The point is to extend this when $n$ is a power of $2$ but also do sublinear time decoding.RIP matrices already work for any universe. I think the way we currently write it is not fair, and might even hurt, also leave the readers consfused.}.


%\Zhao{I can't find a sentence (in text, but not table) that we mentioned the oder of strongness of each guarantees, $\ell_{\infty}/\ell_2$, $\ell_2/\ell_2$, $\ell_2/\ell_1$. We can cite \cite{p14,p16} and also some Eric's paper.}


==> arxiv/libtheorems.tex <==
% Code for theorems in multiple places
% Originally by Eric Price, placed in the public domain
%
% This lets you write the statement of a theorem/lemma in one place
% and insert it in multiple parts of a document.  This lets you
% include the statement of Lemma 3.2 in both the introduction and the
% place that it's proven, and the numbering can refer to the place
% where it's proven.
%
% Usage:
%
%  \define[optional title]{thm:main}{Theorem}{We show \[ x^2 + y^2 \geq 2xy \].}
%     Before you use it.
%
%  \state{thm:main}
%     in the place where you want the label to be generated
%
%  \restate{thm:main}
%     elsewhere.
%
%  To have consistent equation labels, use $\thmlabel{eq:1}$ rather
%  than $\label{eq:1}$.
%
%
%%%%% Begin code
\usepackage{etoolbox}

\makeatletter

% Define the various variables to be used in \state/\restate
\newcommand{\define}[4][ignore]{%
  \ifstrequal{#1}{ignore}{}{
  \@namedef{thmtitle@#2}{#1}}%
  \@namedef{thm@#2}{#4}%
  \@namedef{thmtypen@#2}{lemma}%
  \newtheorem{thmtype@#2}[theorem]{#3}%
  \newtheorem*{thmtypealt@#2}{#3~\ref{#2}}%
}

% State the theorem, generating the proper number.
\newcommand{\state}[1]{%
  \@namedef{curthm}{#1}
  \@ifundefined{thmtitle@#1}{
  \begin{thmtype@#1}
    }{
  \begin{thmtype@#1}[\@nameuse{thmtitle@#1}]
  }
    \label{#1}
    \@nameuse{thm@#1}
  \end{thmtype@#1}
  \@ifundefined{thmdone@#1}{
  \@namedef{thmdone@#1}{stated}%
  }{}
}

% Include the theorem, with the original numbering
\newcommand{\restate}[1]{%
  \@namedef{curthm}{#1}
  \@ifundefined{thmtitle@#1}{
    \begin{thmtypealt@#1}
    }{
  \begin{thmtypealt@#1}[\@nameuse{thmtitle@#1}]
  }
    \@nameuse{thm@#1}
  \end{thmtypealt@#1}
  \@ifundefined{thmdone@#1}{
  \@namedef{thmdone@#1}{stated}%
  }{}
}

% For equations, this generates a new number if this is the first time
% the theorem is included, and reuses the old number otherwise.
\newcommand{\thmlabel}[1]{
  \@ifundefined{thmdone@\@nameuse{curthm}}{\label{#1}
    }{\tag*{\eqref{#1}}}
}
\makeatother
%%%%% End code


==> arxiv/preli.tex <==
\section{Preliminaries}

For any positive integer $n$, we define $\mathbb{Z}_n$ and $\mathbb{Z}_n^*$ as follows:
\begin{align*}
\mathbb{Z}_n = \{ 0, 1 , 2, \cdots , n-1\}, \text{~~~and~~~} \mathbb{Z}_n^* = \{ 1,2, \cdots, n-1 \}.
\end{align*}

We assume that the universe size $n = p^d$ where both $p$ and $d$ are positive integers. 
Let $\omega = e^{2\pi\i / p}$.
We will work with the normalized $d$-dimensional Fourier transform
\begin{align*}
\wh{x}_f = \frac{1}{ \sqrt{n} } \sum_{t \in [p]^d} x_t \cdot \omega^{f^\top t}, & ~ \forall f \in [p]^d
\end{align*}
and the inverse Fourier transform is
\begin{align*}
x_t = \frac{1}{ \sqrt{n} } \sum_{f \in [p]^d} \wh{x}_f \cdot \omega^{-f^\top t}, & ~ \forall t \in [p]^d.
\end{align*}

For any vector $x$ and integer $k$, we denote $x_{-k}$ to be the vector obtained by zeroing out the largest (in absolute value) $k$ coordinates from $x$.


==> arxiv/reduce.tex <==
\section{Reduction}
\Zhao{Write Michael Reduction here}


==> arxiv/tech.tex <==
\subsection{Preliminaries}\label{sec:preliminary}

For any positive integer $n$, we use $[n]$ to denote $\{1,2,\cdots,n\}$. 
We assume that the universe size $n = p^d$ for any positive integer $p$. Our algorithm facilitates $n = \Pi_{j=1}^d p_j$ for any positive integers $p_1,\ldots,p_d$, but we decide to present the case $n=p^d$ for ease of exposition; the proof is exactly the same in the more general case.
Let $\omega = e^{2\pi\i / p}$ where $\i = \sqrt{-1}$.
We will work with the normalized $d$-dimensional Fourier transform
\begin{align*}
\wh{x}_f = \frac{1}{ \sqrt{n} } \sum_{t \in [p]^d} x_t \cdot \omega^{f^\top t}, & ~ \forall f \in [p]^d
\end{align*}
and the inverse Fourier transform is
\begin{align*}
x_t = \frac{1}{ \sqrt{n} } \sum_{f \in [p]^d} \wh{x}_f \cdot \omega^{-f^\top t}, & ~ \forall t \in [p]^d.
\end{align*}

For any vector $x$ and integer $k$, we denote $x_{-k}$ to be the vector obtained by zeroing out the largest (in absolute value) $k$ coordinates from $x$.

\subsection{Our result}


Apart from being dimension-independent and working for any universe size, our algorithm satisfies $\ell_\infty/\ell_2$, which is the strongest guarantee out of the standard guarantees considered in compressed sensing tasks. A guarantee $G_1$ is stronger than guarantee $G_2$ if for any $k$-sparse recovery algorithm that satisfies $G_1$ we can obtain a $O(k)$-sparse recovery algorithm that satisfies $G_2$. See also below for a comparison between $\ell_\infty/\ell_2$ and $\ell_2/\ell_2$, the second stronger guarantee.

Previous work is summarized in Table \ref{tbl:table}. Our result is the following.

\begin{theorem}[main result, informal version]\label{thm:fourier_sparse_recovery_informal}
Let $n = p^d$ where both $p$ and $d$ are positive integers.
Let $x \in \C^{[p]^d}$.
Let $k \in \{1, \ldots, n\}$. 
Assume that $R^* \geq \|\wh{x}\|_\infty / \|\wh{x}_{-k}\|_2$ where $\log R^* = O(\log n)$ (signal-to-noise ratio).
There is an algorithm that takes $O(k \log k \log n)$ samples from $x$, runs in $\wt{O}( n )$ time, and outputs a $O(k)$-sparse vector $y$ such that
\begin{align*}
\| \wh{x} - y \|_{\infty} \leq \frac{1}{\sqrt{k}} \|\wh{x}_{-k}\|_2
\end{align*}
holds with probability at least $1 - 1 / \poly(n)$.
\end{theorem}


\begin{table}[!t]
\centering
  \begin{tabular}{ | l | l | l | l | l | l|}
    \hline
    {\bf Reference} & {\bf Samples} & {\bf Time} & {\bf Filter} & {\bf RIP} & {\bf Guarantee} \\ \hline
    \cite{gms05} & $k \log^{O(d)}n$ & $k \log^{ O(d)} n$ & Yes & No & $\ell_2/\ell_2$ \\ \hline
    \cite{ct06}& $k\log^6 n$ & $\poly(n)$ & No & Yes & $\ell_2/\ell_1$ \\ \hline
    \cite{rv08} & $k \log^2 k \log(k \log n) \log n$ & $\tilde{O}(n)$ & No & Yes & $\ell_2/\ell_1$\\ \hline
    \cite{hikp12a} & $k \log^d n \log (n/k)$ & $k \log^d n \log (n/k)$ & Yes & No & $\ell_2/\ell_2$ \\ \hline
    %\cite{hikp12a} & $k \log^{d+1} n \log (n/k)$ & $k \log^{d+1} n \log (n/k)$ & Yes & No & $\ell_\infty/\ell_2$ \\ \hline
    \cite{cgv13} & $k\log^3 k \log n$ & $\tilde{O}(n)$ & No & Yes & $\ell_2/\ell_1$\\ \hline
    \cite{ik14} & $2^{d \log d} k \log n $ & $\tilde{O}( n)$ & Yes & No & $\ell_{\infty}/\ell_2$ \\ \hline
    \cite{b14} & $k \log k \log^2 n$ & $\tilde{O}(n)$ & No & Yes & $\ell_2/\ell_1$ \\ \hline
    \cite{hr16} & $k\log^2 k \log n$ & $\tilde{O}(n)$ & No & Yes & $\ell_2/\ell_1$ \\ \hline
    \cite{k16,k17} & $2^{d^2} k \log n  $ & $2^{d^2}k \log^{d+O(1)} n $ & Yes & No & $\ell_2/\ell_2$ \\ \hline
    \cite{kvz19} & $k^3 \log^2 k \log^2 n$ & $k^3 \log^2 k \log^2 n$ & Yes & Yes & Exactly $k$-sparse\\ \hline
    Theorem~\ref{thm:fourier_sparse_recovery_informal} & $k \log k \log n$ & $\tilde{O}(n)$ & No & No & $\ell_{\infty}/\ell_2$ \\ \hline
    % Theorem~\ref{thm:fourier_sparse_recovery_optimal} & $k \log n$ if $k = O(\log n)$ & $\tilde{O}(n)$ & No \\ \hline
  \end{tabular}\caption{$n = p^d$. We ignore the $O$ for simplicity. The $\ell_{\infty}/\ell_2$ is the strongest possible guarantee, with $\ell_2/\ell_2$ coming second, $\ell_2/\ell_1$ third and exactly $k$-sparse being the weaker. We also note that all \cite{rv08,cgv13,b14,hr16} obtain improved analyses of the Restricted Isometry property; the algorithm is suggested and analyzed (modulo the RIP property) in \cite{bd08}. 
  The work in \cite{hikp12a} does not explicitly state the extension to the $d$-dimensional case, 
  but can easily be inferred from the arguments. \cite{hikp12a,ik14,k16,kvz19} work when the universe size in each dimension are powers of $2$. 
  We also assume that the signal-to-noise ratio is bounded by a polynomial of $n$, which is a standard assumption in the sparse Fourier transform literature \cite{hikp12a,ik14,k16,k17,ln19}.
} \label{tbl:table}
\end{table}



\paragraph{Comparison between $\ell_\infty/\ell_2$ and $\ell_2/\ell_2$ (or $\ell_2/\ell_1$).}
For the sake of argument, we will consider only the $\ell_2/\ell_2$ guarantee which is stronger than $\ell_2/\ell_1$.
The $\ell_2/\ell_2$ guarantee is the following: for $ \wh{x} \in \mathbb{C}^n$ one should output a $z$ such that $\|\wh{x} - z\|_2 \leq C  \| \wh{x}_{-k} \|_2$, where $C>1$ is the approximation factor. The $\ell_2/\ell_2$ guarantee can be immediatelly obtained by $\ell_\infty/\ell_2$ guarantee by truncating $z$ to its top $k$ coordinates. 
Consider $C=1.1$ \footnote{This is the case with the \textsc{RIP} based approaches, which obtain $\ell_2/\ell_1$. 
In fact, many filter-based algorithms facilitate $(1+\epsilon)$ on the right-hand side, with the number of measurements being multiplied by $\epsilon^{-1}$. 
By enabling the same dependence on $\epsilon^{-1}$ our algorithm facilitates a multiplicative $\epsilon$ factor on the right-hand side of the $\ell_\infty/\ell_2$, which makes it much stronger. Thus, a similar argument can go through.}, and think of the following signal: for a set $S$ of size $0.05k$ we have $|\wh{x}_i| =\frac{2}{\sqrt{k}} \|\wh{x}_{\bar{S}}\|_2$. 
Then the all zeros vectors is a valid solution for the $\ell_2/\ell_2$ guarantee, since 
\begin{align*}
\|\vec 0 - \wh{x}\|_2^2  = \|\wh{x}_S\|_2^2 + \|\wh{x}_{\bar{S}}\|_2^2 =  0.05 k \cdot \frac{4}{ k} \|\wh{x}_{\bar{S}}\|_2^2 + \|\wh{x}_{\bar{S}}\|_2^2 = 1.2\| \wh{x}_{\bar{S}}\|_2^2 < 1.1^2 \|\wh{x}_{\bar{S}}\|_2^2.
\end{align*}


It is clear that since $\vec 0$ is a possible output, we may not recover any of the coordinates in $S$, which is the set of ``interesting'' coordinates. 
On the other hand, the $\ell_{\infty}/\ell_2$ guarantee does allow the recovery of every coordinate in $S$. 
This is a difference between recovering all $0.05k$ versus $0$ coordinates. 
From the above discussion, one can conclude in the case where there is too much noise, $\ell_2/\ell_2$ becomes much weaker than $\ell_\infty/\ell_2$, and can be even meaningless. 
Thus, $\ell_\infty/\ell_2$ is highly desirable, whenever it is possible. 
The same exact argument holds for $\ell_2/\ell_1$.



\begin{remark}
We note that \cite{ct06,rv08,cgv13,b14,hr16} obtain a uniform guarantee, i.e. with $1-1/\mathrm{poly}(n)$ they allow reconstruction of all vectors; $\ell_\infty/\ell_2$ and $\ell_2/\ell_2$ are impossible in the uniform case, see \cite{cdd09}. We note that our comparison between the guarantees is in terms of the quality of approximation. With respect to that, $\ell_\infty/\ell_2$ is the strongest one. 
\end{remark}

\subsection{Summary of previous Filter function based technique}

%\Zhao{
%First describe Count-Sketch?, then describe how filter implement Count-Sketch in FFT setting.

%Then write about 5~10 lines for each Eric/Michael paper? e.g. \cite{hikp12a}, \cite{ik14}, \cite{k16} , \cite{kvz19}. The filters are changing over papers, slightly mention some difference about good filter (\cite{hikp12a}) and crude filter (can't remember which Michael's paper),  }

One of the two ways to perform Fourier sparse recovery is by trying to implement arbitrary linear measurements, with algorithms similar to the ubiquitous \textsc{CountSketch} \cite{ccf02}. 
In the general setting \textsc{CountSketch} hashes every coordinate to one of the $O(k)$ buckets, and repeats $O( \log n)$ times with fresh randomness. 
Then, it is guaranteed that every heavy coordinate will be isolated, and the contribution from non-heavy elements is small. 
To implement this in the Fourier setting becomes a highly non-trivial task however: one gets access only to the time-domain but not the frequency domain. 
One natural way to do this is to exploit the convolution theorem and find a function which is sparse in the time domain and approximates the indicator of an interval (rectangular pulse) in the frequency domain; these functions are called (bandpass) filters. 
Appropriate filters were designed in \cite{hikp12a,hikp12b}: they were very good approximations of the rectangular pulse, i.e. the contribution from elements outside the passband zone contributed only by $1/\poly( n )$ their mass. 
These filters had an additional $\log n$ factor (in one dimension) in the sparsity of the time domain and they are sufficient for the purposes of \cite{hikp12a}, but in high dimensions this factor becomes $\log^d n$. 
Filters based on the Dirichlet kernel give a better dependence in terms of sparsity and dimension (although still an exponential dependence on the latter), but the leak to subsequent buckets, i.e. coordinates outside the passband zone contribute a constant fraction of their mass, in contrast to the filter used in \cite{hikp12a}. 
Thus one should perform additional denoising, which is a non-trivial task. 
The seminal work of Indyk and Kapralov \cite{ik14} was the first that showed how to perform sparse recovery with these filters, and then Kapralov \cite{k16,k17} extended this result to run in sublinear time. 
Note that any filter-based approach with filters which approximate the $\ell_\infty$ box suffers from the curse of dimensionality. 
\cite{kvz19} devised an algorithm which avoids the curse of dimensionality by using careful aliasing, but it works in the noiseless case and has a cubic dependence on $k$. 

\subsection{RIP property-based algorithms: a quick overview}

We say the matrix $A \in \C^{m \times n}$ satisfies RIP (Restricted Isometry Property \cite{ct05}) of order $k$ if for all $k$-sparse vectors $x \in \C^n$ we have $\|A x\|_2^2 \approx \|x \|_2^2$. 
A celebrated result of Candes and Tao \cite{ct06} shows that Basis Pursuit ($\ell_1$ minimization) suffices for sparse recovery, as long as the samples from the time domain satisfy RIP. 

In \cite{ct06} it was also proved using generic chaining that random sampling with oversampling factor $O(\log^6 n)$ gives RIP property for any orthonormal matrix with bounded entries by $1/\sqrt{n}$. 
Then \cite{rv08} improved the bound to $O(k \cdot \log^2 k \cdot \log (k \log n) \cdot \log n)$ and \cite{cgv13} improved it to $O(k \cdot \log^3k \cdot \log n)$. 
Subsequent improvement by Bourgain \cite{b14} has lead to $O(k \log k \cdot \log^2 n)$ samples, improved by Haviv and Regev to $O(k \log^2 k \cdot \log n)$\cite{hr16}. 
The fastest set of algorithms are iterative ones: for example Iterative Hard Thresholding \cite{bd09} or CoSaMP \cite{nt09} run in $O(\log n)$ iterations\footnote{To be precise, their running time is logarithmic in the signal-to-noise ratio.} and each iteration takes $\wt{O}(n)$ time. 



We note the recent lower bound of \cite{r19}: a subsampled Fourier matrix that satisfies the RIP properties should have $\Omega(k \log k \cdot d)$ rows\footnote{\cite{bllm19} independently gives a similar bound for $d=\log n$.}. 
This bound is particularly useful in high dimensions, since it deteriorates to a trivial bound in low dimensions. 
We still believe though that a bound of $\Omega( k \log k \log n)$ should hold in all dimensions. 
Thus, what remains is to obtain the $\ell_2/\ell_2$ guarantee by giving a tighter analysis, and removing the one $\log k$ factor to match the lower bound, but our algorithm already allows Fourier sparse recovery with these number of samples, even with a stronger guarantee. 


\subsection{Overview of our technique}

Let $x \in \C^{[p]^d}$ denote our input signal in the time domain. 
In the following we assume the knowledge of $\mu = \frac{1}{\sqrt{k}}\|\wh{x}_{-k}\|_2$ and $R^*$ which is an upper bound of $\|\wh{x}\|_\infty / \mu$, and bounded by $\poly( n )$.
These are standard assumption \cite{hikp12a,ik14,k16,k17,ln19} in the sparse Fourier transform literature. 
The bound on $R^*$ is useful for bounding the running time (or the number of measurements in \cite{hikp12a}) and in any of \cite{hikp12a,ik14,k16,k17,ln19} a $\log n$ can be substituted by $\log R^*$ in the general case, which is also the case for our algorithm. 
We note that our algorithm will be correct with probability $1-1/\poly(n)$ whenever $R^* < 2^{n^{100}}$; this is fine for every reasonable application. It might seem counter-intuitive that we need this upper bound on $R^*$, since intuitively larger signal to noise ratio should only help. However, this is an artifact of the techniques of Sparse Fourier Transform in general, either they are iterative or not.
We assumed the rounding errors in FFT computation to be negligible, similarly to Remark 3.4 in \cite{ik14}.

\subsubsection{Estimators and random shifts}

Consider the simplest scenario: $d=1$, $p$ is a prime number and a $1$-sparse signal $\wh{x}$ which is $1$ on some frequency $f^*$. 
From a sample $x_t$ in the time-domain what would be the most reasonable way to find $f^*$? For every $f \in [p]$ we would compute 
\begin{align*}
\sqrt{n} \omega^{ft}x_t = \sqrt{n} \omega^{ft} \cdot \frac{1}{\sqrt{n}} \sum_{f'\in [p]} \omega^{-f't} \wh{x}_{f'} = \omega^{(f-f^*)t},
\end{align*}
and keep, for $ t\neq 0$, the frequency that gives a real number. 
Since $(f-f^*)t$ will be zero only for $ f= f^*$, we are guaranteed correct recovery. In the noisy and multi-dimensional case or $p$ is an arbitrary integer, however, this argument will not work, because of the presence of contribution from other elements and the fact that $(f-f^*)^\top t$ can be zero modulo $p$ for other frequencies apart from $f$. 
However, we can take a number of samples $t$ and average $\sqrt{n}\omega^{f^\top t}$, and hope that this will make the contribution from other frequencies small enough, so that we can infer whether $f$ corresponds to a heavy coordinate or not. 
More specifically, we pick a set $T$ of frequencies uniformly at random from $[p]^d$ and compute
\begin{align*}
\frac{\sqrt{n}}{|T|}\sum_{t \in T} \omega^{f^\top t }x_t 
\end{align*}
for all frequencies $f$. 
We show that if $|T| = O(k)$ our estimator is good on average (and later we will maintain $O(\log n)$ independent instances and take the median to make sure with probability $1 - 1 / \poly(n)$ the estimators for all the frequencies are good), and in fact behaves like a crude filter, similarly to the ones used in \cite{ik14}, in the sense that every coordinate contributes a non-trivial amount to every other coordinate. 
However, these estimators do not suffer from the curse of dimensionality and our case is a little bit different, requiring a quite different handling. 
The main reason is that in contrast to the filters used in \cite{ik14}, there is not an easy way to formulate an isolation argument from heavy elements that would allow easy measurement re-use, like Definition 5.2 and Lemma 5.4 from \cite{ik14}. 
Buckets induced by filter functions have a property of locality, since they correspond to approximate $\ell_\infty$ boxes (with a polynomial decay outside of the box) in $[p]^d$: the closer two buckets are the more contribute the elements of one into the other. 
Our estimators on the other side do not enjoy such a property. 
Thus, one has to proceed via a different argument. 

In what follows, we will discuss how to combine the above estimators with an iterative loop that performs denoising, i.e. removes the contribution of every heavy element to other heavy elements.

\paragraph{Random shifts.} Our approach for performing denoising is quite general, and is clean on a high-level. Let $S$ be the set of the large coordinates of $\wh{x}$, i.e. those with magnitude at least $(1/\sqrt{k}) \|\wh{x}_{-k}\|_2$. We are going to estimate $\wh{x}_f$ for $f \in [p]^d$ using the estimators introduced in the previous paragraphs. Then, for those frequencies $f$ for which the values obtained are sufficiently large (larger than $\|x\|_\infty\cdot 2^{-\ell}$) , we are going to implicitly subtract that value from $\wh{x}_f$; this corresponds to updating the signal, a common trick in the Sparse Fourier literature. Then we shall iterate, re-using the same samples again till the signal to noise ratio becomes small enough. It can be shown that only coordinates in $S$ are ever updated. The trick for sample reuse in our case is the following: in the $\ell$th iteration we approximate $\mathbb{C}^{[p]^d}$ by an appropriate grid of side length $\beta\|x\|_\infty\cdot 2^{-\ell}$, where $\beta$ is an absolute constant, and then keep $O(\log n)$ random shifts of it.  Keeping $O(\log n)$ randomly shifted grids one can show that in every iteration a nice property is satisfied: we can guarantee that there exists a grid such that for all $f \in S$, $\wh{x}_f$ and its estimator round to the same point. Projecting onto that grid, what our algorithm shows is that the signal under update follows a predictable trajectory, something that allows us to argue about the correctness of the algorithm without taking an intractable union-bound over all possible trajectories the algorithm could evolve. In essence, our algorithm shows that we can at $\ell$th step compute every $\wh{x}_f$ up to $\|\wh{x}\|_\infty 2^{-\ell}$ error.  

\paragraph{A high-level explanation.}
Let us try to combine the previous two ideas. Assume that at iteration $\ell$ we have an approximation of $\wh{x}_f$ for all $f \in S$ up to $\|x\|_{\infty}\cdot 2^{-\ell}$. If we were to pick $O(k \log n \log k)$ fresh samples, we could, using our estimators, approximate $\wh{x}_f$ up to $(1/k) \|x\|_{\infty}\cdot 2^{-\ell}$. Let that approximation be $y$. We then round $y$ to $O(\log n)$ randomly shifted grids of diameter $ \|x\|_{\infty}\cdot 2^{-\ell}$. A probabilistic argument shows that, due to our choice of parameters, with high probability there exists a grid such that $\wh{x}_f$ and $y_f$ are rounded to the same grid point (the additional $O(\log k)$ factor in the sample complexity is what makes this argument go through); and we can also decide which grid this is! Thus, we safely project $y$ and be sure that what we now have at our hands is $\wh{x}$ projected onto that grid. Thus, in the next iteration $\ell+1$ we only need to argue correctness for at most $O(\log n)$ vectors, that is, vectors $\wh{x}$ rounded on one of the aforementioned $O(\log n)$ grids. This dramatically decreases the number of events we have to analyze, and we can set up an inductive argument that guarantees the correctness of the algorithm. Note that there is no independence issue, since the randomness between the samples taken (used for the estimators) and the projection onto the randomly shifted grids is not shared.\newline


We first implement a procedure which takes $O(k \log n)$ uniform random measurements from $x$ and has the guarantee that for any $\nu \geq \mu$ any $y \in \C^{[p]^d}$ where $\|\wh{x} - y \|_\infty \leq 2 \nu$ and $y$ is independent from the randomness of the measurements, the procedure outputs a $O(k)$-sparse $z \in \C^{[p]^d}$ such that $\|\wh{x} - y - z\|_\infty \leq \nu$ with probability $1 - 1 / \poly(n)$. 

\begin{lemma} [\textsc{LinfinityReduce} procedure, informal]\label{lem:locate_and_estimate_informal}
Let $\mu = \frac{1}{\sqrt{k}} \|\wh{x}_{-k}\|_2$, and $\nu \geq \mu$.
Let ${\cal T}^{(0)}$ be a list of $O(k \log n)$ i.i.d. elements in $[p]^d$. 
Let $S$ be top $O(k)$ coordinates in $\wh{x}$. %, where $C_S = 26$.
There is a procedure that takes $\{x_t\}_{t \in {\cal T}}$, $y \in \C^{[p]^d}$ and $\nu$ as input, runs in $\wt{O}(n)$ time, and outputs $z \in \C^{[p]^d}$ so that if $\| \wh{x} - y \|_\infty \leq 2 \nu$, 
$\supp(y) \subseteq S$ and $y$ is independent from the randomness of ${\cal T}^{(0)}$, then $\| \wh{x} - y - z \|_\infty \leq \nu$ and $\supp(z) \subseteq S$ with probability $1 - 1 / \poly(n)$ under the randomness of ${\cal T}^{(0)}$.
\end{lemma}



Namely, we can take $O(k \log n)$ measurements and run the procedure in Lemma~\ref{lem:locate_and_estimate_informal} to reduce (the upper bound of) the $\ell_\infty$ norm of the residual signal by half.
We call the procedure in Lemma~\ref{lem:locate_and_estimate_informal} \textsc{LinfinityReduce} procedure.
More generally, we can take $O(H \cdot k \log n)$ measurements and run the \textsc{LinfinityReduce} procedure $H$ times to reduce the $\ell_\infty$ norm of the residual signal to $1 / 2^H$ of its original magnitude, with failure probability at most $1 / \poly(n)$.
Note that if we set $H = \log R^*$, we have already obtained a 
m taking $O(k \log n \log R^*)$ measurements, because we can drive down (the upper bound of) the $\ell_\infty$ norm of the residual signal from $\|\wh{x}\|_\infty$ to $\mu$ in $\log R^*$ iterations. 

% \begin{comment}
\subsubsection{$O(k \log n)$ samples for $k = O(\log n)$}\label{sec:warmup}
We first discuss a measurement reuse idea that leads us to a sparse recovery algorithm (Algorithm~\ref{alg:fourier_sparse_recovery_k_logn}) taking $O(k \log n)$ measurements for $k = O(\log n)$.
We set $H = 5$, and let ${\cal T} = \{{\cal T}^{(1)}, \ldots, {\cal T}^{(H)}\}$, where each ${\cal T}^{(h)}$ is a list of $O(k \log n)$ i.i.d. elements in $[p]^d$.
Note that ${\cal T}^{(1)}, \ldots, {\cal T}^{(H)}$ are independent.
In our sparse Fourier recovery algorithm, we will measure $x_t$ for all $t \in {\cal T}$.


In a nutshell, our approach finely discretizes the space of possible trajectories the algorithm could evolve, and carefully argues about the correctness of the algorithm by avoiding the intractable union-bound over all trajectories.

\paragraph{Recovery algorithm.} The recovery algorithm proceeds in $\log R^* - H + 1$ iterations, where each iteration (except the last iteration) the goal is to reduce the upper bound of $\ell_\infty$ norm of the residual signal by half. 
Initially, the upper bound is $R^*$.
It is important to note that we use the same measurements ${\cal T} = \{{\cal T}^{(1)}, \ldots, {\cal T}^{(H)}\}$ in all of these $\log R^* - H + 1$ iterations.

In the following, we will describe one iteration of the recovery algorithm. 
Let $y \in \C^{[p]^d}$ denote the sparse vector recovered so far, and let the upper bound of $\|\wh{x} - y\|_\infty$ be $2 \nu$. 
Running the \textsc{LinfinityReduce} procedure $H$ times where in the $h$-th time we use measurements in ${\cal T}^{(h)}$, we obtain a $O(k)$-sparse $z$ such that with probability $1 - 1 / \poly(n)$, $\|\wh{x} - y - z\|_\infty \leq 2^{1-H} \nu \leq 0.1 \nu$ (we call such $z$ a desirable output by the \textsc{LinfinityReduce} procedure).
Instead of taking $y+z$ as our newly recovered sparse signal, for each $f \in \supp(y+z)$, we project $y_f+z_f$ to the nearst points in $\mathcal{G}_{0.6 \nu}:= \{0.6 \nu (x + y \i): x,y \in \Z \}$ and assign to $y'_f$, where $y'$ denotes our newly recovered sparse signal.
For all $f \not\in \supp(y+z)$, we let $y'_f = 0$.

To simplify our exposition, here we introduce some notations.
We call $\mathcal{G}_{0.6 \nu}$ a grid of side length $0.6 \nu$, and we generalize the definition to any side length.
Namely, for any $r_g > 0$, let grid $\mathcal{G}_{r_g}:= \{r_g(x + y \i): x,y \in \Z \}$.
Moreover, we define $\Pi_{r_g}: \C \rightarrow \mathcal{G}_{r_g}$ to be the mapping that maps any element in $\C$ to the nearest element in $\mathcal{G}_{r_g}$.
Now we can write $y'$ as
\begin{align*}
y'_f = 
\begin{cases} 
  \Pi_{0.6 \nu}(y_f + z_f), & \text{~if~} f \in \supp(y+z); \\ 
  0, & \text{~if~} f \not\in \supp(y+z).
\end{cases} 
\end{align*}

At the end of each iteration, we assign $y'$ to $y$, and shrink $\nu$ by half. In the last iteration, we will not compute $y'$, instead we output $y+z$. 
We present the algorithm in Algorithm~\ref{alg:fourier_sparse_recovery_k_logn}.

\begin{algorithm}[!t]\caption{Fourier sparse recovery by projection, $O(k \log n)$ measurements when $k = O(\log n)$}\label{alg:fourier_sparse_recovery_k_logn}
\begin{algorithmic}[1]
\Procedure{\textsc{FourierSparseRecoveryByProjection}}{$x,n,k,\mu,R^*$} \Comment{Section~\ref{sec:warmup}} 
  \State {\bf Require} that $\mu = \frac{1}{\sqrt{k}} \|\wh{x}_{-k}\|_2$ and $R^* \geq \|\wh{x}\|_\infty\ / \mu$ 
  \State $H \leftarrow 5$, $\nu \leftarrow \mu R^* / 2$, ~$y \leftarrow \vec 0$ \Comment{$y \in \C^{[p]^d}$ refers to the sparse vector recovered so far}
  \State Let ${\cal T} = \{ {\cal T}^{(1)}, \cdots, {\cal T}^{(H)} \}$ where each ${\cal T}^{(h)}$ is a list of i.i.d. uniform samples in $[p]^d$ 
  \While {{\bf true}} 
    \State $\nu' \leftarrow 2^{1-H} \nu$
    \State Use $\{x_t\}_{t\in \mathcal{T}}$ to run the \textsc{LinfinityReduce} procedure (in Lemma~\ref{lem:locate_and_estimate_informal}) $H$ times (use samples in ${\cal T}^{(h)}$ for each $h\in [H]$ ), and finally it finds $z$ so that $\|\wh{x} - y - z\|_\infty \leq \nu'$ 
    \State{{\bf if} {$\nu' \leq \mu$} } {\bf then} \Return $y+z$ \Comment{We found the solution}
    \State $y' \leftarrow \vec 0$
    \For{$f \in \supp(y+z)$}
      \State $y'_f \leftarrow \Pi_{0.6 \nu}(y_f + z_f)$ \Comment{We want $\|\wh{x} - y' \|_\infty \leq \nu$ and the depend-}
    \EndFor \Comment{ence between $y'$ and $\mathcal{T}$ is under control~~~}
    \State $y \leftarrow y'$, $\nu \leftarrow \nu / 2$
  \EndWhile
\EndProcedure
\end{algorithmic}
\end{algorithm}

\paragraph{Analysis.} We analyze $y'$ conditioned on the event that $\|\wh{x} - y - z\|_\infty \leq 0.1 \nu$ (i.e. $z$ is a desirable output by the \textsc{LinfinityReduce} procedure, which happens with probability $1 - 1 / \poly(n)$).
We will prove that $y'$ has two desirable properties: (1) $\|\wh{x} - y'\|_\infty \leq \nu$; (2) the dependence between $y'$ and our measurements ${\cal T}$ is under control so that after taking $y'$ as newly recovered sparse signal, subsequent executions of the \textsc{LinfinityReduce} procedure with measurements ${\cal T}$ still work with good probability. 
Property (1) follows from triangle inequality and the fact that $\|\wh{x} - (y+z)\|_\infty \leq 0.1 \nu$ and $\|(y+z) - y'\|_\infty \leq 0.6 \nu$.
We now elaborate on property (2). 
We can prove that for any $f \in [p]^d$, 
\begin{align*}
y'_f \in \big\{\Pi_{0.6\nu}(\wh{x}_f+0.1\nu(\alpha+ \beta\i)): \alpha, \beta \in \{-1, 1\} \big\}.
\end{align*}
Let $S$ denote top $26 k$ coordinates (in absolute value) of $\wh{x}$.
We can further prove that for any $f \in \ov{S}$, $y'_f =0$.
Therefore, the total number of possible $y'$ is upper bounded by $4^{|S|} = 4^{O(k)}$.
If $k = O(\log n)$, we can afford union bounding all $4^{O(k)} = \poly(n)$ possible $y'$, and prove that with probability $1 - 1 / \poly(n)$ for all possible value of $y'$ if we take $y'$ as our newly recovered sparse signal then in the next iteration the \textsc{LinfinityReduce} procedure with measurements ${\cal T}$ gives us a desirable output.

\paragraph{Sufficient event.}
More rigorously, we formulate the event that guarantees successful execution of Algorithm~\ref{alg:fourier_sparse_recovery_k_logn}.
Let ${\cal E}_1$ be the event that for all $O(\log R^*)$ possible values of $\nu \in \{ \mu \frac{ R^*}{2}, \mu \frac{ R^*}{4}, \ldots, \mu 2^{H-1} \}$,
for all possible vector $y$ where $y_f = 0$ for $f \in \ov{S}$ and $y_f \in \{ \Pi_{0.6 \nu} (\wh{x}_f + 0.1 \nu(\alpha + \beta \i)): \alpha, \beta \in \{-1, 1\} \}$ for $f \in S$ (we also need to include the case that $y = \vec 0$ for the success of the first iteration), 
running the \textsc{LinfinityReduce} procedure (in Lemma~\ref{lem:locate_and_estimate_informal}) $H$ times (where in the $h$-th time measurements $\{x_t\}_{t \in {\cal T}^{(h)}}$ are used to reduce the error from $2^{2-h} \nu$ to $2^{1-h} \nu$) finally gives $z$ so that $\|\wh{x} - y - z\|_\infty \leq 2^{1-H} \nu$.
The randomness of ${\cal E}_1$ comes from ${\cal T} = \{ {\cal T}^{(1)}, \ldots, {\cal T}^{(H)} \}$.

First, event ${\cal E}_1$ happens with probability $1 - 1 / \poly(n)$. This is because there are $4^{O(k)} \log R^*$ possible combinations of $\nu$ and $y$ to union bound, and each has failure probability at most $1 / \poly(n)$.
For $k = O(\log n)$, and any $R^* < 2 ^{n^{100}}$ this gives the desired result.
Second, conditioned on event ${\cal E}_1$ happens, Algorithm~\ref{alg:fourier_sparse_recovery_k_logn} gives correct output.
This can be proved by a mathematical induction that in the $t$-th iteration of the while-true loop in Algorithm~\ref{alg:fourier_sparse_recovery_k_logn}, $\|\wh{x} - y\|_\infty \leq 2^{-t} \mu R^*$.

% \end{comment}
\subsubsection{$O(k \log k\log n)$ samples suffice}

We first introduce some notations.
For any $r_g > 0$, define the grid $\mathcal{G}_{r_g}:= \{r_g(x + y \i): x,y \in \Z \}$.
Moreover, we define $\Pi_{r_g}: \C \rightarrow \mathcal{G}_{r_g}$ to be the mapping that maps any element in $\C$ to the nearest element in $\mathcal{G}_{r_g}$.

\begin{comment}
At every iteration, our algorithm holds a vector $y$, and computes a vector $z$. Instead of setting $y$ to $y+z$ and iterating, as would be the natural thing to do, we set $y$ to $y'$ where
\begin{align*}
y'_f = 
\begin{cases} 
  \Pi_{0.6 \nu}(y_f + z_f), & \text{~if~} f \in \supp(y+z); \\ 
  0, & \text{~if~} f \not\in \supp(y+z).
\end{cases} 
\end{align*}
\end{comment}

\paragraph{Using random shift to reduce projection size.}


%We remark that in the analysis of the previous recovery algorithm, if we can make sure that every $y_f+z_f$ has only one possible outcome when projecting to the grid $\mathcal{G}_{0.6 \nu}$, then we no longer need to union bound $4^{O(k)}$ events.
%However, if $\wh{x}_f$ is very close to a grid point in ${\cal G}_{0.6 \nu}$ (or $\wh{x}_f \in {\cal G}_{0.6 \nu}$), then no matter how close $y_f+z_f$ and $\wh{x}_f$ are, $\Pi_{0.6 \nu}(y_f + z_f)$ will have $4$ possible values.

We introduce the random shift trick, the property of which is captured by Lemma~\ref{lem:random_shift_informal}. To simplify notation, for any $r_b > 0$ and $c \in \C$ we define box $\mathcal{B}_\infty(c, r_b) := \{c + r_b(x+y \i): x,y \in [-1,1]\}$.
For any $S \subseteq \C$, let $\Pi_{r_g}(S) = \{\Pi_{r_g}(c) : c \in S\}$.

\begin{lemma} [property of a randomly shifted box, informal] \label{lem:random_shift_informal} % restatement of Lemma~\ref{lem:random_shift}
Take a box of side length $2r_b$ and shift it randomly by an offset in $\mathcal{B}_\infty(0, r_s)$ (or equivalently, $[-r_s, r_s] \times [-r_s, r_s]$) where $r_s \geq r_b$. Next round every point inside that shifted box to the closest point in $G_{r_g}$ where $r_g \geq 2 r_s$. Then, with probability at least $(1 - r_b/r_s)^2$ everyone will be rounded to the same point.
\end{lemma}

In the following, we present a sparse Fourier recovery algorithm that incorporates the random shift idea.
The algorithm takes $O(k \log k \log n)$ measurements. We set $H = O(\log k)$ and take measurements of ${\cal T} = \{{\cal T}^{(1)}, \ldots, {\cal T}^{(H)}\}$ , where ${\cal T}^{(h)}$ is a list of $O(k \log n)$ i.i.d elements in $[p]^d$. 
%Note that ${\cal T}^{(1)}, \ldots, {\cal T}^{(H)}$ are independent, and the choice of $H$ is different from Section~\ref{sec:warmup}.

In a nutshell, our approach finely discretizes the space of possible trajectories the algorithm could evolve. After we find estimates for $\wh{x}_f$ we shift them randomly and project them onto a coarse grid (which is the same as projecting onto one of randomly shifted grids). We shall show that then the number of trajectories is pruned, and we need to argue for a much smaller collection of events.
We note that we make the decoding algorithm randomized: the randomness in previous algorithms was present only when taking samples, and the rest of the algorithm was deterministic. However, here we need randomness in both cases, and that helps us prune the number of possible trajectories. To the best of our knowledge, this is a novel argument and approach, and might be helpful for future progress in the field.


\paragraph{Recovery algorithm.} We assume that we have already obtained a $O(k)$-sparse $y \in \C^{[p]^d}$ such that $\|\wh{x} - y\|_\infty \leq 2 \nu$ and $y$ is ``almost'' independent from ${\cal T}$.
We show how to obtain $y' \in \C^{[p]^d}$ such that $\|\wh{x} - y'\|_\infty \leq \nu$ with probability $1 - 1 / \poly(n)$ and $y'$ is ``almost'' independent from ${\cal T}$.
The idea is the following. We first run the \textsc{LinfinityReduce} procedure $H = O(\log k)$ times to get an $O(k)$-sparse $z \in \C^{[p]^d}$ such that $\|\wh{x} - y - z\|_\infty \leq \frac{1}{2^{20}k} \nu$.
Then we repeatedly sample a uniform random shift $s \in [- 10^{-3} \nu,  10^{-3} \nu] + \i  [-10^{-3} \nu,  10^{-3} \nu]$ until for every $f \in \supp(y+z)$, all the points (or complex numbers) of the form $y_f + z_f +s + a + b \i$ with $a,b \in [-\frac{\nu}{2^{20}k}, \frac{\nu}{2^{20}k}]$ round to the same grid point in $\mathcal{G}_{0.04 \nu}$.
Finally, for every $f \in \supp(y+z)$, we assign $\Pi_{0.04 \nu} (y_f + z_f + s)$ to $y'_f$; all remaining coordinates in $y'$ will be assigned $0$.
We present an informal version of our algorithm in Algorithm~\ref{alg:fourier_sparse_recovery_informal}, and defer its formal version to the appendix.

\begin{algorithm}[!t]\caption{Fourier sparse recovery by random shift and projection (informal version)}\label{alg:fourier_sparse_recovery_informal} % formal version in Algorithm~\ref{alg:fourier_sparse_recovery}
\begin{algorithmic}[1]
\Procedure{\textsc{FourierSparseRecovery}}{$x,n,k,\mu,R^*$} \Comment{Theorem~\ref{thm:fourier_sparse_recovery_informal}, $n=p^d$} 
  \State {\bf Require} that $\mu = \frac{1}{\sqrt{k}} \|\wh{x}_{-k}\|_2$ and $R^* \geq \|\wh{x}\|_\infty\ / \mu$
  \State $H \leftarrow O(\log k)$, $\nu \leftarrow \mu R^* / 2$, ~$y \leftarrow \vec 0$ \Comment{$y \in \C^{[p]^d}$ refers to the sparse vector recovered so far}
  \State  Let ${\cal T} = \{ {\cal T}^{(1)}, \cdots, {\cal T}^{(H)} \}$ where each ${\cal T}^{(h)}$ is a list of i.i.d. uniform samples in $[p]^d$ 
  \While {{\bf true}} 
    \State $\nu' \leftarrow \frac{1}{2^{20}k} \nu$
    \State Use $\{x_t\}_{t\in \mathcal{T}}$ to run the \textsc{LinfinityReduce} procedure (in Lemma~\ref{lem:locate_and_estimate_informal}) $H$ times (use samples in ${\cal T}^h$ for each $h\in [H]$ ), and finally it finds $z$ so that $\|\wh{x} - y - z\|_\infty \leq \nu'$ 
    \State{{\bf if} {$\nu' \leq \mu$} } {\bf then} \Return $y+z$ \Comment{We found the solution}
    \Repeat %\Comment{{\it Randomized decoding procedure}}
      \State Pick $s \in \mathcal{B}_\infty(0, 10^{-3}\nu)$ uniformly at random \label{lin:s_informal}
    \Until{$\forall f \in \supp(y+z), |\Pi_{0.04 \nu}(\mathcal{B}_\infty(y_f + z_f + s, \nu'))|=1$} \label{lin:until_good_informal}
    \State $y' \leftarrow \vec 0$	\label{lin:start_project}
    \For{$f \in \supp(y+z)$}
      \State $y'_f \leftarrow \Pi_{0.04 \nu}(y_f + z_f + s)$ \Comment{We want $\|\wh{x} - y' \|_\infty \leq \nu$ and the depend-}
    \EndFor \Comment{ence between $y'$ and $\mathcal{T}$ is under control~~~} 
    \State $y \leftarrow y'$, $\nu \leftarrow \nu / 2$ \label{lin:end_project}
  \EndWhile
\EndProcedure
\end{algorithmic}
\end{algorithm}

\paragraph{Informal Analysis.} We analyze the above approach.

At every iteration, our algorithm holds a vector $y$, and computes a vector $z$. Instead of setting $y$ to $y+z$ and iterating, as would be the natural thing to do, we set $y$ to $y'$ (lines \ref{lin:start_project} to \ref{lin:end_project}) where
\begin{align*}
y'_f = 
\begin{cases} 
  \Pi_{0.6 \nu}(y_f + z_f), & \text{~if~} f \in \supp(y+z); \\ 
  0, & \text{~if~} f \not\in \supp(y+z).
\end{cases} 
\end{align*}


First, we have the guarantee that $\|\wh{x} - y'\|_\infty \leq \nu$.
Moreover, by our choice of $s$, for every $f \in \supp(y+z)$, $y_f + z_f + s$ and $\wh{x}_f + s$ round to the same grid point in $\mathcal{G}_{0.04 \nu}$. 
Therefore, for the new vector $y'$ we have recovered, we ``hide'' the randomness in ${\cal T}$, and the randomness only leaks from failed attempts of the shifts.
In the following, we show that each attempt of shift succeeds with probability $\frac{1}{2}$.

We can restate the procedure of choosing $s$ to be: 
\begin{align*}
\text{{\bf repeatedly}} & ~ \text{~sample~} s \sim \mathcal{B}_\infty(0, 10^{-3}\nu), \\
\text{{\bf until}} & ~ \text{~for~all~} f \in \supp(y+z), \Big|\Pi_{0.04\nu} \Big( \mathcal{B}_\infty \big( y_f + z_f +s, \frac{\nu}{2^{20}k} \big) \Big) \Big| = 1.
\end{align*}
Note that $|\supp(y+z)| = O(k)$. 
Let us say that we can always guarantee that $|\supp(y+z)| \leq 50 k$.
By Lemma~\ref{lem:random_shift_informal} where we let $r_b = \frac{\nu}{2^{20}k}$, $r_s = 10^{-3} \nu$ and $r_g = 0.04 \nu$, for $f \in \supp(y+z)$,% the probability that 
\begin{align*}
\Pr \Bigg[ \Big| \Pi_{0.04\nu} \left( \mathcal{B}_\infty \big(y_f + z_f +s, \frac{\nu}{2^{20}k} \big) \right) \Big| = 1 \Bigg] \geq \left(1 - \frac{r_b}{r_s}\right)^2 \geq 1 - \frac{1}{100k}.
\end{align*}
By a union bound over $f \in \supp(y + z)$, the probability is at least $\frac{1}{2}$ that for all $f \in \supp(y+z)$, $|\Pi_{0.04\nu}(\mathcal{B}_\infty(y_f + z_f +s, \frac{\nu}{2^{20}k}))| = 1$.

Therefore, with probability $1 - 1 / \poly(n)$, we will only try $O(\log n)$ shifts.
We can apply a union bound over $O(\log n)$ possible shifts, and prove that with probability $1 - 1 / \poly(n)$ if taking $y'$ as our new $y$, and shrinking $\nu$ by half, the \textsc{LinfinityReduce} procedure will work as desired as if there is no dependence issue.

\paragraph{Sufficient event.}
Let $S$ be top $O(k)$ coordinates in $\wh{x}$ which are also larger than $(1/\sqrt{k}) \|x_{-k}\|_2$ in magnitude.
Let $L = O(\log R^*)$ denote the number of iterations in Algorithm~\ref{alg:fourier_sparse_recovery_informal}.
For $\ell \in [L]$, let $\nu_\ell = 2^{-\ell} \mu R^*$.
For $\ell \in [L-1]$, let $s_\ell^{(a)}$ be the $a$-th sample from $\mathcal{B}_\infty(0, 10^{-3} \nu_\ell)$ as appeared on Line~\ref{lin:s_informal} in Algorithm~\ref{alg:fourier_sparse_recovery_informal}.
For the sake of analysis, we assume that Algorithm~\ref{alg:fourier_sparse_recovery_informal} actually produces an infinite sequence of shifts $s_\ell^{(1)}, s_\ell^{(2)}, \ldots$.
We formulate the event that guarantees successful execution of Algorithm~\ref{alg:fourier_sparse_recovery_informal}.
We define event $\mathcal{E}_2$ to be the union of all the following events. \\
1. For all $\ell \in [L-1]$, there exists $a \in [10 \log n]$ so that for all $f \in S$,
\begin{align*}
\left| \Pi_{0.04 \nu_\ell} \left(\mathcal{B}_\infty(\wh{x}_f + s_\ell^{(a)}, \frac{1}{100k} \nu_\ell) \right) \right| = 1.
\end{align*} 
\\
2. For $\ell = 1$, if we run the \textsc{LinfinityReduce} procedure $H$ times with $y = \vec 0$ and measurements in ${\cal T}$, we get $z$ such that $\|\wh{x} - z\|_\infty \leq 2^{1-H} \nu_1$ and $\supp(z) \subseteq S$. \\
3. For all $\ell \in \{2, \ldots, L\}$, for all $a \in [10 \log n]$, if we run the \textsc{LinfinityReduce} procedure $H$ times with $y = \xi$ where
\begin{align*}
\xi_f = 
\begin{cases} 
  \Pi_{0.04 \nu_\ell}(\wh{x}_f + s_{\ell-1}^{(a)}), & \text{~if~} f \in S; \\ 
  0, & \text{~if~} f \in \ov{S}.
\end{cases} 
\end{align*}
then we get $z$ such that $\|\wh{x} - y - z\|_\infty \leq 2^{1-H} \nu_\ell$  and $\supp(y+z) \subseteq S$.

We can prove that event ${\cal E}_2$ happens with probability $1 - 1 / \poly(n)$.
Moreover, we can prove that conditioned on event ${\cal E}_2$ Algorithm~\ref{alg:fourier_sparse_recovery_informal} gives correct output.
We defer both proofs in the appendix.





% \paragraph{Handling sequence of random shifts}


==> arxiv/towards_optimal.tex <==
\subsection{$O(k \log n)$ measurements if $k = O(\log n)$} \label{sub:fourier_sparse_recovery_optimal}

If $k = O(\log n)$, we can prove that $O(k \log n)$ measurements is enough.
We don't need to use random shifts, though we will still project onto the grid.
When we cannot decide the exact grid point each $\wh{x}_i$ maps to, we are able to choose an adjacent one.
We can afford union-bounding all $9^k$ possible rounding results when $k = O(\log n)$.

\begin{theorem} \label{thm:fourier_sparse_recovery_optimal}
Let $n$ be a prime number.
We assume that $k = O(\log n)$.
There is an algorithm that takes $O(k \log n)$ samples from $x$, runs in $\tilde{O}(n)$ time, and outputs a $k$-sparse vector $z$ such that
\begin{align*}
\| z - \wh{x} \|_2 \leq O(1) \min_{k-\sparse~x_k} \| x_k - \wh{x} \|_2
\end{align*}
holds with probability at least $9/10$.
\end{theorem}

\begin{corollary}
Let $n = p^d$ where $p$ is a prime number.
Assume that $k = O(\log n)$.
There is an algorithm that takes $O(k \log n)$ samples from $x$, runs in $\tilde{O}(n)$ time, and outputs a $k$-sparse vector $z$ such that
\begin{align*}
\| z - \wh{x} \|_2 \leq O(1) \min_{k-\sparse~x_k} \| x_k - \wh{x} \|_2
\end{align*}
holds with probability at least $9/10$.
\end{corollary}


==> arxiv/trash.tex <==
\section{Preliminaries}

TODO :
\begin{itemize}
	\item Copy some definition of Gaussian and Pulse from \cite{hikp12a} or \cite{ps15}
\end{itemize}

Given two vectors $a,b$, we define $a*b$ to be the convolution of $a$ and $b$, i.e., $(a*b)_i = \sum_j a_j b_{i-j}$; we define $a \odot b$ to be the entry-wise product, i.e., $(a \odot b)_i = a_i \cdot b_i$.


Let $I = [-k/2,k/2]$ and $B,C$ sets in $[-n/2,n/2]$ for $n$ much larger than $k$. We define vector $1_B$ to denote the vector such that $(1_B)_i = 1$ if $i\in B$ and $(1_B)_i = 0$ otherwise. We want to approximate $(1_B * 1_C) \odot 1_I$.

\textbf{idea}:

Look at $( 1_B \odot f ) * ( 1_C \odot g )$, the $i$-th entry of which is
\begin{align*}
\sum_{j=-n/2}^{n/2} (1_B)_j \cdot f_j \cdot (1_C)_{i-j} \cdot g_{i-j}.	
\end{align*}
One easy fact we know is
\begin{fact}
Given four vectors $a,b,c,d$, we have
\begin{align*}
(a \odot b) * (c \odot d) = (a * c) \odot ( b * d )
\end{align*}
\end{fact}
\begin{proof}
For each $i$, we have
\begin{align*}
\LHS = & ~ ( (a \odot b) * (c \odot d) )_i \\
= & ~ \sum_j (a \odot b)_j \cdot ( c \odot d )_{i-j} \\
= & ~ \sum_j a_j b_j c_{i-j} d_{i-j} \\
= & ~ ??? \\
= & ~ ( \sum_j a_j c_{i-j} ) \cdot ( \sum_j b_j d_{i-j} ) \\
= & ~ ( a * c )_i \cdot ( b * d )_i \\
= & ~ ( ( a * c ) \odot ( b * d ) )_i \\
= & ~ \RHS
\end{align*}
\end{proof}

Using the above fact, we have
\begin{align*}
( 1_B \odot f ) * ( 1_C \odot g ) = (1_B * 1_C) \odot (f * g). %(1_B * 1_C) \odot I
\end{align*}

If the following two things hold,

\begin{itemize}
\item For $|i| > k \log^c k$, $\sum_{j \in [-n/2,n/2] } f_j g_{i-j} < 1/(2k^2)$.
\item For $|i| \leq k/2$ and all $j$, $f_j g_{i-j} \geq 1/k$, (-> $(f*g)_i \geq 1$)  
\end{itemize}
(\Zhao{it means in \cite{hikp12a} }, $n/(2B) = k$; $f * g \approx I$)
then we are done. 
Can we find such functions $f$ and $g$? Possibly for $f$ to be the discrete Gaussian distribution, and $g$ to be the indicator of $I$, that would work.


%roughly $m^{1-\delta}$ subproblems, each problem has three sets $B,C,I$, $|B| = |C| = |I| = m^{\delta}$.

Originally, the way how they solved it, is using additive combinatorics.
We don't use additive combinatorics.

(Zhao : i don't know how to implement this step.)The running time is $m^{2-O(\delta)}$, our goal is $m^{2-\delta}$

Compute $(1_B * 1_C) \odot 1_I$, 
computing $(1_B * 1_C)$ either takes $n \log n$ time or $k^2$ time. $|B|=|C|=|I|=k$.

$f * g$ approximate $1_I$ ($f * g$ Fourier filter function)

\begin{comment}
1)
if $|i| > 1 \cdot n$, $(f * g)_i \in +/- \delta$
if $|i| \in \alpha/2, 1$, $(f * g)_i \in [0,1] $
if $|i| < \alpha/2 \cdot n$, $(f * g)_i \in 1 +/- \delta$ 

2)
if $i \leq 1 \cdot n$, $(1_I)_i = 1$
else $(1_I)_i = 0$

\end{comment}
$(1_B * 1_C) \odot 1_I 
\approx 
(1_B * 1_C) \odot (f * g) 
\approx
(1_B \odot f) * (1_C \odot g)$,
(location Fourier set query has the definition of $f$ and $g$)

\subsection{Important tricks used in previous sparse FT paper}

\subsubsection{Subsampled FFT}
In \cite{hikp12b}, it mentioned a trick called ``subsampled FFT''. Suppose we have a vector $x \in \C^n$ and a parameter $B$ dividing $n$, and would like to compute $\wh{y}_i = \wh{x}_{ i ( n / B ) }$ for $i \in [B]$.

\begin{claim}[Claim 3.7 in \cite{hikp12b}]
Let vector $y \in \C^B$ be defined as follows : for each $i \in [B]$, $y_i = \sum_{j=0}^{n/B-1} x_{i+ B j}$. Let $\wh{y}$ denote the Fourier transform of $y$.

Therefore $\wh{y}$ can be computed in $O( | \supp(x) | + B \log B )$ time.
\end{claim}
\begin{proof}
Let $\omega = e^{2\pi \i / n}$
We have
\begin{align*}
\wh{x}_{ i (n/B) } = & ~ \sum_{j = 0}^{n-1} x_j \omega^{ij (n/B)} & \text{~by~} \wh{x} = \textsc{FT}(x) \\
= & ~ \sum_{a = 0}^{B-1} \sum_{j = 0}^{n/B-1} x_{ B j + a } \omega^{i (B j + a) n/B} \\
= & ~ \sum_{a = 0}^{B-1} \sum_{j = 0}^{n/B-1} x_{ B j + a } \omega^{i a n / B} & \text{~by~} \omega^{ijn} = 1 \\
= & ~ \sum_{a = 0}^{B-1} y_a \omega^{i a n / B} & \text{~by~} \sum_{j = 0}^{n/B-1} x_{ B j + a } = y_a \\
= & ~ \wh{y}_i . & \text{~by~} \wh{y} = \textsc{FT}(y)
\end{align*}
\end{proof}

\subsubsection{Semi-equispaced Fourier Transform}

See Section 12, page 42 of \url{https://theory.epfl.ch/kapralov/papers/fourier-measurements.pdf}.

\begin{algorithm}[h]\caption{}
\begin{algorithmic}[1]
\Procedure{\textsc{SemiEquispaceFFT}}{$x,c$}
	\State Round $k$ up to a factor of $n$
	\State $G, \wh{G'} \leftarrow \textsc{Filters}(n,k,c)$
	\State $y_i \leftarrow \frac{1}{ \sqrt{n} } ( x * G )_{i n / 2k} $ for $i \in [2k]$
	\State $\wh{y} \leftarrow \textsc{FFT}(y)$
	\State $\wh{x}_i' \leftarrow \wh{y}_i$ for $|i| \leq k / 2$
	\State \Return $\wh{x}'$
\EndProcedure
\end{algorithmic}
\end{algorithm}


\subsection{Filter function}


\subsubsection{Continuous version}
We define rect and sinc function as follows:
\begin{definition}[page 12 in \cite{ckps16}]
\begin{align*}
\sinc (t) = \frac{ \sin ( \pi t ) }{ \pi t }
\end{align*}
\end{definition}

\begin{fact}[continuous version, fact 3.3 in \cite{ckps16}]
We define
\begin{align*}
\rect_s(t) = 
\begin{cases}
1, & \text{~if~} |t| \leq \frac{s}{2}; \\
0, & \text{~otherwise}.
\end{cases}
\end{align*}
Then Fourier transform a of $\rect_s(t)$ is $\wh{\rect_s}(f) = \frac{ \sin( \pi f s ) }{ \pi f s} = \sinc(f s)$.
\end{fact}

Note that \cite{ckps16} used continuous filter function $G(t), \wh{G}(f)$ \footnote{\url{https://arxiv.org/pdf/1609.01361.pdf}, page 79.}. Here we use discrete filter function,
\begin{definition}[continuous version, definition C.11 in \cite{ckps16}]
\begin{align*}
G(t) = & ~ b_0 \cdot ( \rect_{s_1} ( t ) )^{* l} \cdot \sinc ( s_2 t ), \\
\wh{G}_f = & ~ b_0 \cdot ( \sinc ( s_1 f ) )^{\cdot l} * \rect_{s_2} ( f ).
\end{align*}
\end{definition}

\subsubsection{Discrete version}

We can make the discrete version,
\begin{definition}[discrete version]
We define
\begin{align*}
G_i = & ~ b_0 \cdot ( \rect_{s_1} ( i ) )^{* l} \cdot \sinc ( s_2 i ), \forall i \in [n] \\
\wh{G}_i = & ~ b_0 \cdot ( \sinc ( s_1 i ) )^{\cdot l} * \rect_{s_2} ( i ), \forall i \in [n].
\end{align*}
\end{definition}

\begin{lemma} [Properties of the $\sinc$ function, Appendix C in \cite{ckps16}] \label{lem:sinc_property}
% \begin{enumerate}
% \item $\forall t \in \R, 1 - \frac{(\pi t)^2}{3!} \leq \sinc(t) \leq 1$.
% \item $\forall |t| \leq 1.2 / \pi, \sinc(t) \leq 1 - t^2 / 8$. 
% Looks like the above two are not useful here
% \item 
\begin{align*}
\forall |t| > 1.2 / \pi, |\sinc(t)| \leq \frac{1}{\pi |t|}.
\end{align*}
% \end{enumerate}
\end{lemma}

\newpage
% \Zhao{I think we need to compute the following thing. Zhengyu, can you do that?}
\Zhengyu{I tried to adapt the following proof from \cite{ckps16}. Please check if it looks OK.}
\begin{claim}
For each $|i| \leq k/2$, we have
\begin{align*}
\wh{G}_i \in [ 1 - \delta, 1].
\end{align*}
For each $|i| \geq k \log^c k$, we have
\begin{align*}
\wh{G}_i \in [-\delta, \delta].
\end{align*}
\end{claim}

\begin{proof}
By definition of $\wh{G}$, we can rewrite
\begin{align*}
\wh{G}_i = & ~ \sum_{j=1}^n b_0 \cdot ( \sinc (s_1 j) )^{l} \cdot \rect_{s_2} (i - j) \\
= & ~ \sum_{ j \in [i-s_2/2, i+s_2/2] } b_0 \cdot ( \sinc (s_1 j) )^{l}
\end{align*}
The choice for $s_1$, $s_2$, $l$ ($l$ is even number) should be
\begin{align*}
s_1 = \frac{2B}{\alpha n}, ~~~ s_2 = \frac{n}{4B}, ~~~ l = \Omega( \log (k/\delta) )
\end{align*}
For $\alpha$, the choice should $[1/10,9/10]$. 
For $B$, the choice should be $\Theta(n/k)$, since $\Theta(n/B) = k$.
For $b_0$, the choice should be $\Theta(s_1 \sqrt{l}) = \Theta(B \sqrt{l}/ (\alpha n ))$ since we hope $\wh{G}(0) =1$.
Let $s_1 = \beta_1 / k$, and by definition of $s_1$ we have $\beta_1 = \Theta(1)$.
We require that $s_2 \geq (\frac{2}{\beta_1} + 1) k$. In addition, we require $\frac{s_1 s_2}{2}$ is an integer, in order to make subsequent arguments go through.
\Zhengyu{Please check if the above two additional assumptions make any trouble.}

We first prove that 
\begin{align}	
\sum_{j = k/\beta_1}^{\infty} b_0 (\sinc(s_1 j))^l \leq \delta / 2, \label{eq:sinc_tail_sum}
\end{align}

which follows from
\begin{align*}
\sum_{j = k/\beta_1}^{\infty} b_0 (\sinc(s_1 j))^l = & ~ b_0 \sum_{j = k/\beta_1}^{\infty} (\sinc(\beta_1 j / k))^l \\
\leq & ~ b_0 \sum_{j = k/\beta_1}^{\infty} \frac{1}{(\pi \beta_1 j / k)^l} \\
= & ~ b_0 \pi^{-1} \sum_{t = 1}^{\infty} \sum_{j = t k /\beta_1}^{(t+1) 
\frac{k}{\beta_1} - 1} \frac{1}{(\beta_1 j / k)^l} \\
\leq & ~ b_0 \pi^{-l} \sum_{t = 1}^{\infty} \left( \frac{k}{\beta_1} \cdot \frac{1}{t^{l}} \right) \\
= & ~ b_0 \pi^{-l} \cdot \frac{k}{\beta_1} \cdot \sum_{t = 1}^{\infty} \frac{1}{t^{l}} \\
\leq & ~ \delta / 2,
\end{align*}

where the second step follows from Lemma~\ref{lem:sinc_property}, and the last step follows by $l = \Omega(\log (k / \delta))$ and our choice of $b_0 = \Theta(\frac{\sqrt{l}}{k})$.

\noindent
(1) For $|i| \leq k/2$. We will first prove that $\wh{G}_i \leq \wh{G}_0$.
We assume that $0 < i \leq k/2$. The case that $-k/2 \leq i < 0$ is symmetric.

\begin{align*}
\wh{G}_0 - \wh{G}_i = & ~ \sum_{j=-s_2/2}^{s_2/2} b_0 \cdot ( \sinc (s_1 j) )^{l} - \sum_{j = i-s_2/2}^{i+s_2/2} b_0 \cdot ( \sinc (s_1 j) )^{l} \\
= & ~ \sum_{j=-s_2/2}^{i-s_2/2} b_0 \cdot ( \sinc (s_1 j) )^{l} - \sum_{j = s_2/2}^{i+s_2/2} b_0 \cdot ( \sinc (s_1 j) )^{l} \\
= & ~ \sum_{t = 0}^{i} b_0 \cdot ( \sinc (s_1 (t - s_2 / 2)) )^{l} - \sum_{t=0}^{i} b_0 \cdot ( \sinc (s_1 (t + s_2 / 2)) )^{l} \\
= & ~ \sum_{t = 0}^{i} b_0 \cdot ( \sinc (s_1 (-t + s_2 / 2)) )^{l} - \sum_{t=0}^{i} b_0 \cdot ( \sinc (s_1 (t + s_2 / 2)) )^{l} \\
= & ~ b_0 \sum_{t = 0}^{i} \left( ( \sinc (s_1 (-t + s_2 / 2)) )^{l} - ( \sinc (s_1 (t + s_2 / 2)) )^{l} \right) \\
= & ~ b_0 \sum_{t = 0}^{i} \left( \frac{|\sin(\pi s_1 s_2 / 2 - \pi s_1 t)|^l}{(\pi s_1 (-t + s_2/2))^l} - \frac{|\sin(\pi s_1 s_2 / 2 + \pi s_1 t)|^l}{(\pi s_1 (t + s_2/2))^l} \right) \\
= & ~ b_0 \sum_{t=0}^{i} \frac{|\sin(\pi s_1 t)|^l}{(\pi s_1)^l} \left( \frac{1}{(-t+s_2/2)^l} - \frac{1}{(t+s_2/2)^l} \right) \\
\geq & ~ 0,
\end{align*}

where the forth step follows by the function $\sinc(\cdot )^l$ is an even function because $l$ is an even integer, the seventh step follows by $\frac{s_1s_2}{2}$ is an integer, and the last steps follows by $|-t + s_2/2| \leq |t + s_2/2|$. By our choice of $b_0$, we have $\wh{G}_0 = 1$. Therefore, $\wh{G}_i \leq 1$.

Now we will prove that $\wh{G}_i \geq 1 - \delta$.
Note that by our assumption that $s_2 \geq (\frac{2}{\beta_1}+1)k$, we have $\frac{s_2}{2} - \frac{k}{2} \geq \frac{k}{\beta_1}$. 
For $|i| \leq \frac{k}{2}$, we have $i-\frac{s_2}{2}-1 \leq \frac{k}{2} - \frac{s_2}{2} -1 \leq -\frac{k}{\beta_1}$ and $i+\frac{s_2}{2}+1 \geq \frac{k}{2} + \frac{s_2}{2} + 1 \geq \frac{k}{\beta_1}$.
Therefore,

\begin{align*}
\wh{G}_i = & ~ \sum_{j=-\infty}^{\infty} b_0 \cdot ( \sinc (s_1 j) )^{l} - \sum_{j=-\infty}^{i - s_2/2 - 1} b_0 \cdot ( \sinc (s_1 j) )^{l} - \sum_{j = i + s_2/2 + 1}^{\infty} b_0 \cdot ( \sinc (s_1 j) )^{l} \\
\geq & ~ \sum_{j=-k/2}^{k/2} b_0 \cdot ( \sinc (s_1 j) )^{l} - \sum_{j=-\infty}^{-k / \beta_1} b_0 \cdot ( \sinc (s_1 j) )^{l} - \sum_{j = k / \beta_1}^{\infty} b_0 \cdot ( \sinc (s_1 j) )^{l} \\
= & ~ 1 - 2 \sum_{j = k / \beta_1}^{\infty} b_0 \cdot ( \sinc (s_1 j) )^{l} \\
\geq & ~ 1 - \delta,
\end{align*}

where the last step follows from \eqref{eq:sinc_tail_sum}.

\noindent
(2) For $|i| \geq k\log^c k$, we can bound $\wh{G}_i$:
\begin{align*}
\wh{G}_i = & ~ b_0 \sum_{j = i-s_2/2}^{i+s_2/2} (\sinc(\beta_1 j / k))^l \\
\leq & ~ b_0 \sum_{j = k / \beta_1}^{\infty} (\sinc(\beta_1 j / k))^l \\
< & ~ \delta,
\end{align*}
where the second step follows by $s_2 = \Theta(k)$ and $|i| \geq k \log^c k$ so that $i - s_2/2 \geq k / \beta_1$, and the third step follows by \eqref{eq:sinc_tail_sum}.

\end{proof}


\subsection{New filter}

\Zhao{Billy, can you write down the property of the filter (you think will work), first? Then we can discuss how to construct the filter.}


\begin{comment}
Let $I$ denote a continuous size $k$ set. Let $B$, $C$ denote two $k$-sparse vectors, let $G$ denote the Gaussian filter, and $P$ denote the rectangular filter. Roughly speaking $G * P \approx I$. We define vector $z$ as follows:
\begin{align*}
z = ( B \cdot G ) * ( C \cdot P )
\end{align*}
We want to prove two things : \\
1. If $|i| < k/2$, then $z_i$ is large \\
2. If $|i| > k$, then $z_i$ is small

One fact we know is
\begin{align*}
( B \cdot G ) * ( C \cdot P ) = (B * C) \cdot ( G * P ).
\end{align*}
\end{comment}


==> arxiv/warmup.tex <==
\section{$O(k \log n)$ measurements for $k = O(\log n)$}\label{sec:warmup}
We first discuss a measurement reuse idea that leads us to a sparse recovery algorithm (Algorithm~\ref{alg:fourier_sparse_recovery_k_logn}) taking $O(k \log n)$ measurements for $k = O(\log n)$.
We set $H = 5$, and let ${\cal T} = \{{\cal T}^{(1)}, \ldots, {\cal T}^{(H)}\}$, where each ${\cal T}^{(h)}$ is a list of $O(k \log n)$ i.i.d. elements in $[p]^d$.
Note that ${\cal T}^{(1)}, \ldots, {\cal T}^{(H)}$ are independent.
In our sparse Fourier recovery algorithm, we will measure $x_t$ for all $t \in {\cal T}$.


In a nutshell, our approach finely discretizes the space of possible trajectories the algorithm could evolve, and carefully argues about the correctness of the algorithm by avoiding the intractable union-bound over all trajectories.

\paragraph{Recovery algorithm.} The recovery algorithm proceeds in $\log R^* - H + 1$ iterations, where each iteration (except the last iteration) the goal is to reduce the upper bound of $\ell_\infty$ norm of the residual signal by half. 
Initially, the upper bound is $R^*$.
It is important to note that we use the same measurements ${\cal T} = \{{\cal T}^{(1)}, \ldots, {\cal T}^{(H)}\}$ in all of these $\log R^* - H + 1$ iterations.

In the following, we will describe one iteration of the recovery algorithm. 
Let $y \in \C^{[p]^d}$ denote the sparse vector recovered so far, and let the upper bound of $\|\wh{x} - y\|_\infty$ be $2 \nu$. 
Running the \textsc{LinfinityReduce} procedure $H$ times where in the $h$-th time we use measurements in ${\cal T}^{(h)}$, we obtain a $O(k)$-sparse $z$ such that with probability $1 - 1 / \poly(n)$, $\|\wh{x} - y - z\|_\infty \leq 2^{1-H} \nu \leq 0.1 \nu$ (we call such $z$ a desirable output by the \textsc{LinfinityReduce} procedure).
Instead of taking $y+z$ as our newly recovered sparse signal, for each $f \in \supp(y+z)$, we project $y_f+z_f$ to the nearst points in $\mathcal{G}_{0.6 \nu}:= \{0.6 \nu (x + y \i): x,y \in \Z \}$ and assign to $y'_f$, where $y'$ denotes our newly recovered sparse signal.
For all $f \not\in \supp(y+z)$, we let $y'_f = 0$.

To simplify our exposition, here we introduce some notations.
We call $\mathcal{G}_{0.6 \nu}$ a grid of side length $0.6 \nu$, and we generalize the definition to any side length.
Namely, for any $r_g > 0$, let grid $\mathcal{G}_{r_g}:= \{r_g(x + y \i): x,y \in \Z \}$.
Moreover, we define $\Pi_{r_g}: \C \rightarrow \mathcal{G}_{r_g}$ to be the mapping that maps any element in $\C$ to the nearest element in $\mathcal{G}_{r_g}$.
Now we can write $y'$ as
\begin{align*}
y'_f = 
\begin{cases} 
  \Pi_{0.6 \nu}(y_f + z_f), & \text{~if~} f \in \supp(y+z); \\ 
  0, & \text{~if~} f \not\in \supp(y+z).
\end{cases} 
\end{align*}

At the end of each iteration, we assign $y'$ to $y$, and shrink $\nu$ by half. In the last iteration, we will not compute $y'$, instead we output $y+z$. 
We present the algorithm in Algorithm~\ref{alg:fourier_sparse_recovery_k_logn}.

\begin{algorithm}[!t]\caption{Fourier sparse recovery by projection, $O(k \log n)$ measurements when $k = O(\log n)$}\label{alg:fourier_sparse_recovery_k_logn}
\begin{algorithmic}[1]
\Procedure{\textsc{FourierSparseRecoveryByProjection}}{$x,n,k,\mu,R^*$} \Comment{Section~\ref{sec:warmup}} 
  \State {\bf Require} that $\mu = \frac{1}{\sqrt{k}} \|\wh{x}_{-k}\|_2$ and $R^* \geq \|\wh{x}\|_\infty\ / \mu$ 
  \State $H \leftarrow 5$, $\nu \leftarrow \mu R^* / 2$, ~$y \leftarrow \vec 0$ \Comment{$y \in \C^{[p]^d}$ refers to the sparse vector recovered so far}
  \State Let ${\cal T} = \{ {\cal T}^{(1)}, \cdots, {\cal T}^{(H)} \}$ where each ${\cal T}^{(h)}$ is a list of i.i.d. uniform samples in $[p]^d$ 
  \While {{\bf true}} 
    \State $\nu' \leftarrow 2^{1-H} \nu$
    \State Use $\{x_t\}_{t\in \mathcal{T}}$ to run the \textsc{LinfinityReduce} procedure (in Lemma~\ref{lem:locate_and_estimate_informal}) $H$ times (use samples in ${\cal T}^{(h)}$ for each $h\in [H]$ ), and finally it finds $z$ so that $\|\wh{x} - y - z\|_\infty \leq \nu'$ 
    \State{{\bf if} {$\nu' \leq \mu$} } {\bf then} \Return $y+z$ \Comment{We found the solution}
    \State $y' \leftarrow \vec 0$
    \For{$f \in \supp(y+z)$}
      \State $y'_f \leftarrow \Pi_{0.6 \nu}(y_f + z_f)$ \Comment{We want $\|\wh{x} - y' \|_\infty \leq \nu$ and the depend-}
    \EndFor \Comment{ence between $y'$ and $\mathcal{T}$ is under control~~~}
    \State $y \leftarrow y'$, $\nu \leftarrow \nu / 2$
  \EndWhile
\EndProcedure
\end{algorithmic}
\end{algorithm}

\paragraph{Analysis.} We analyze $y'$ conditioned on the event that $\|\wh{x} - y - z\|_\infty \leq 0.1 \nu$ (i.e. $z$ is a desirable output by the \textsc{LinfinityReduce} procedure, which happens with probability $1 - 1 / \poly(n)$).
We will prove that $y'$ has two desirable properties: (1) $\|\wh{x} - y'\|_\infty \leq \nu$; (2) the dependence between $y'$ and our measurements ${\cal T}$ is under control so that after taking $y'$ as newly recovered sparse signal, subsequent executions of the \textsc{LinfinityReduce} procedure with measurements ${\cal T}$ still work with good probability. 
Property (1) follows from triangle inequality and the fact that $\|\wh{x} - (y+z)\|_\infty \leq 0.1 \nu$ and $\|(y+z) - y'\|_\infty \leq 0.6 \nu$.
We now elaborate on property (2). 
We can prove that for any $f \in [p]^d$, 
\begin{align*}
y'_f \in \big\{\Pi_{0.6\nu}(\wh{x}_f+0.1\nu(\alpha+ \beta\i)): \alpha, \beta \in \{-1, 1\} \big\}.
\end{align*}
Let $S$ denote top $26 k$ coordinates (in absolute value) of $\wh{x}$.
We can further prove that for any $f \in \ov{S}$, $y'_f =0$.
Therefore, the total number of possible $y'$ is upper bounded by $4^{|S|} = 4^{O(k)}$.
If $k = O(\log n)$, we can afford union bounding all $4^{O(k)} = \poly(n)$ possible $y'$, and prove that with probability $1 - 1 / \poly(n)$ for all possible value of $y'$ if we take $y'$ as our newly recovered sparse signal then in the next iteration the \textsc{LinfinityReduce} procedure with measurements ${\cal T}$ gives us a desirable output.

\paragraph{Sufficient event.}
More rigorously, we formulate the event that guarantees successful execution of Algorithm~\ref{alg:fourier_sparse_recovery_k_logn}.
Let ${\cal E}_1$ be the event that for all $O(\log R^*)$ possible values of $\nu \in \{ \mu \frac{ R^*}{2}, \mu \frac{ R^*}{4}, \ldots, \mu 2^{H-1} \}$,
for all possible vector $y$ where $y_f = 0$ for $f \in \ov{S}$ and $y_f \in \{ \Pi_{0.6 \nu} (\wh{x}_f + 0.1 \nu(\alpha + \beta \i)): \alpha, \beta \in \{-1, 1\} \}$ for $f \in S$ (we also need to include the case that $y = \vec 0$ for the success of the first iteration), 
running the \textsc{LinfinityReduce} procedure (in Lemma~\ref{lem:locate_and_estimate_informal}) $H$ times (where in the $h$-th time measurements $\{x_t\}_{t \in {\cal T}^{(h)}}$ are used to reduce the error from $2^{2-h} \nu$ to $2^{1-h} \nu$) finally gives $z$ so that $\|\wh{x} - y - z\|_\infty \leq 2^{1-H} \nu$.
The randomness of ${\cal E}_1$ comes from ${\cal T} = \{ {\cal T}^{(1)}, \ldots, {\cal T}^{(H)} \}$.

First, event ${\cal E}_1$ happens with probability $1 - 1 / \poly(n)$. This is because there are $4^{O(k)} \log R^*$ possible combinations of $\nu$ and $y$ to union bound, and each has failure probability at most $1 / \poly(n)$.
For $k = O(\log n)$, and any $R^* < 2 ^{n^{100}}$ this gives the desired result.
Second, conditioned on event ${\cal E}_1$ happens, Algorithm~\ref{alg:fourier_sparse_recovery_k_logn} gives correct output.
This can be proved by a mathematical induction that in the $t$-th iteration of the while-true loop in Algorithm~\ref{alg:fourier_sparse_recovery_k_logn}, $\|\wh{x} - y\|_\infty \leq 2^{-t} \mu R^*$.

==> dis.tex <==
\newpage
\section{Some Not So Useful Discussions}
\Zhao{This section probably has nothing to do with our main result for optimal sample $d$-dimensional Fourier transform. We can ignore it for now, and remove it later.}

We will assume that $x(t) = x^*(t) + g(t)$, and $x^*(t)$ has a $k$-sparse Fourier representation.

We will need the following lemma.

\begin{lemma} \label{lem:primes}
Pick $ R = c \log k $ primes in $[ C k \log (FT), 2C k \log (FT) ]$. Let this set be $P$. Then, for any $S \subseteq \{ -FT, \ldots -1, 0, 1 , \ldots , FT\}$ of $k$ elements, we have that the following holds with $1- 1/k$ probability.

For every $x \in S$ there exist at least $2R/3$ primes in $P$ such that $x \neq y \pmod p$ for every $ y \in S \setminus \{x\}$.
\end{lemma}

\begin{proof}(Sketch)
By the prime number theorem, there exist $\beta k \log (FT) / (\log k + \log\log FT)$ primes in that interval, where $\beta$ is at least $\frac{C}{\log C}$. 
% \Zhengyu{to be more exact, there are $\Theta( k \log (FT) / (\log k + \log\log FT))$ primes. If $\log\log FT = \omega(\log k)$, then the number of primes is not what you wrote.}
For all $x,y \in \{ -FT, \ldots -1, 0, 1 , \ldots , FT\}$, we have that $x - y$ can have at most $\alpha \log (FT) / (\log k + \log\log FT)$ prime factors in that interval, for some constant $\alpha$.

Thus, for fixed $x,y$ the probability that a random prime in $[ C k \log (FT), 2C k \log (FT) ]$ divides $x-y$ is upper bounded by 
\begin{align*}
\frac{\alpha \log (FT) / (\log k + \log\log FT)}{\beta k \log (FT) / (\log k + \log\log FT)} = \frac{\alpha}{\beta} \frac{1}{k} \leq \frac{1}{10k},
\end{align*}
where the last step follows from $\beta \geq \frac{C}{\log C}$ and $C$ is sufficiently large.
Thus, for fixed $x \in S$, with constant probability a random prime will not divide anyone in the set $\{ x-y: y \in S \setminus \{x\} \}$. 
By Chernoff bound, if we are taking $R = c \log k$ random primes for large enough $c$, then with probability $1 - 1/\poly(k)$, at least $\frac{2}{3} R$ of them will not divide any element in the set $\{ x-y: y \in S \setminus \{x\} \}$.
A union bound on all $x \in S$ concludes the lemma.  
% \Zhao{I don't understand the meaning of $ x - ( S \setminus \{ x \} )$}
\end{proof}


We will also need the next Lemma.

\begin{lemma} \label{lem:alias}
Let $y$ be a signal with $k$-sparse Fourier representation
\begin{align*}
	y(t) = \sum_{ j= 1}^k v_j e^{2\pi \iu f_j t }.
\end{align*}
Let $\wh{z}$ denote the $p$-dimensional Fourier transform of the vector
$z$ with $z_j = y(j / ( \eta p) )$. Then, % \Zhao{$z_j = y_{ j / (\eta p) }$ ?} %the result is a vector the $i$th coordinate of which equals
\begin{align*}
\wh{z}_i = \sum_{ j : (f_j/\eta) = i \pmod p} v_j.
\end{align*}
\end{lemma}

\begin{proof}
\begin{align*}
\wh{z}_i = & ~ \frac{1}{p} \sum_{s = 1} ^ {p} e^{-2 \pi \iu s i /p} z_s \\
= & ~ \frac{1}{p} \sum_{s = 1} ^ {p} e^{-2 \pi \iu s i /p} y(s/(\eta p)) \\
= & ~ \frac{1}{p} \sum_{s = 1} ^ {p} e^{-2 \pi \iu s i /p} \sum_{j = 1} ^ {k} v_j e^{2 \pi \iu f_j s / (\eta p)} \\
= & ~ \frac{1}{p} \sum_{j = 1} ^ {k} v_j \sum_{s = 1} ^ {p} e^{2 \pi \iu f_j s / (\eta p) - 2 \pi \iu s i /p} \\
= & ~ \frac{1}{p} \sum_{j = 1} ^ {k} v_j \sum_{s = 1} ^ {p} e^{2 \pi \iu \frac{s}{p} (\frac{f_j}{\eta} - i)} \\
\end{align*}
\Zhengyu{If $\frac{f_j}{\eta}$ is an integer, then $\sum_{s = 1} ^ {p} e^{2 \pi \iu \frac{s}{p} (\frac{f_j}{\eta} - i)} = 1_{(f_j/\eta) = i \pmod p}$. But what if $\frac{f_j}{\eta}$ is not an integer?}
\Vasileios{ Let us fix firs t the case that $f_j$ are multiples of $C \eta$, for some constant $C$}
\end{proof}


Now, which is the idea? Take the $R$ random primes, and consider signal $x$ with Lemma~\ref{lem:alias} and all these random primes. For most primes the $v_j$ will be isolated, hence you can read them. Call these samples Set $1$. Consider also $y(t - 1)$, which has Fourier transform by the shift Theorem,
\begin{align*}
y(t - 1) = \sum_{j=1}^k \left(v_j e^{-2\pi f_j} \right) \cdot e^{2 \pi f_j t }. 
\end{align*}

Using Lemma \ref{lem:alias} and the above observation, as well as the samples from Set $1$, we can infer the $f_j$.

\begin{lemma} \label{lem:alias_2}
Consider signal $x'(t) = x^*(t+1)$. Let $\hat{w}$ denote the $p$-dimensional Fourier transform of the vector $w$ with $w_j = x'(j/(\eta p))$. Then,
\begin{align*}
	\hat{w}_i = \sum_{ j : (f_j/\eta) = i \pmod p} e^{2 \i \pi f_j} v_j.	
\end{align*}
%\Zhao{What is $w'$? I don't understand the summation. I don't understand $e^{2\pi f_j} v_j$ also, should it be $e^{2\pi \i f_j t} v_j$ or $e^{2\pi \i f_j}$?}
\end{lemma}

Using Lemma \ref{lem:alias} and \ref{lem:alias_2} with the primes from Lemma \ref{lem:primes}  we can find $v_j$ and $f_j$ in $O( k \log (FT) \log k)$ sample and time. The duration is $O(1/\eta)$, and we can perfectly reconstruct the signal if $g = 0$.

\begin{comment}
\begin{algorithm}
\begin{algorithmic}
\Procedure{aa}{}
	\State
\EndProcedure
\end{algorithmic}
\end{algorithm}
\end{comment}


==> preli.tex <==
\section{Preliminaries}

For any positive integer $n$, we define $\mathbb{Z}_n$ and $\mathbb{Z}_n^*$ as follows:
\begin{align*}
\mathbb{Z}_n = \{ 0, 1 , 2, \cdots , n-1\}, \text{~~~and~~~} \mathbb{Z}_n^* = \{ 1,2, \cdots, n-1 \}.
\end{align*}

We assume that the universe size $n = p^d$ where both $p$ and $d$ are positive integers. 
Let $\omega = e^{2\pi\i / p}$.
We will work with the normalized $d$-dimensional Fourier transform
\begin{align*}
\wh{x}_f = \frac{1}{ \sqrt{n} } \sum_{t \in [p]^d} x_t \cdot \omega^{f^\top t}, & ~ \forall f \in [p]^d
\end{align*}
and the inverse Fourier transform is
\begin{align*}
x_t = \frac{1}{ \sqrt{n} } \sum_{f \in [p]^d} \wh{x}_f \cdot \omega^{-f^\top t}, & ~ \forall t \in [p]^d.
\end{align*}

For any vector $x$ and integer $k$, we denote $x_{-k}$ to be the vector obtained by zeroing out the largest (in absolute value) $k$ coordinates from $x$.


==> reduce.tex <==
\section{Reduction}
\Zhao{Write Michael Reduction here}


==> towards_optimal.tex <==
\subsection{$O(k \log n)$ measurements if $k = O(\log n)$} \label{sub:fourier_sparse_recovery_optimal}

If $k = O(\log n)$, we can prove that $O(k \log n)$ measurements is enough.
We don't need to use random shifts, though we will still project onto the grid.
When we cannot decide the exact grid point each $\wh{x}_i$ maps to, we are able to choose an adjacent one.
We can afford union-bounding all $9^k$ possible rounding results when $k = O(\log n)$.

\begin{theorem} \label{thm:fourier_sparse_recovery_optimal}
Let $n$ be a prime number.
We assume that $k = O(\log n)$.
There is an algorithm that takes $O(k \log n)$ samples from $x$, runs in $\tilde{O}(n)$ time, and outputs a $k$-sparse vector $z$ such that
\begin{align*}
\| z - \wh{x} \|_2 \leq O(1) \min_{k-\sparse~x_k} \| x_k - \wh{x} \|_2
\end{align*}
holds with probability at least $9/10$.
\end{theorem}

\begin{corollary}
Let $n = p^d$ where $p$ is a prime number.
Assume that $k = O(\log n)$.
There is an algorithm that takes $O(k \log n)$ samples from $x$, runs in $\tilde{O}(n)$ time, and outputs a $k$-sparse vector $z$ such that
\begin{align*}
\| z - \wh{x} \|_2 \leq O(1) \min_{k-\sparse~x_k} \| x_k - \wh{x} \|_2
\end{align*}
holds with probability at least $9/10$.
\end{corollary}


==> trash.tex <==
\section{Preliminaries}

TODO :
\begin{itemize}
	\item Copy some definition of Gaussian and Pulse from \cite{hikp12a} or \cite{ps15}
\end{itemize}

Given two vectors $a,b$, we define $a*b$ to be the convolution of $a$ and $b$, i.e., $(a*b)_i = \sum_j a_j b_{i-j}$; we define $a \odot b$ to be the entry-wise product, i.e., $(a \odot b)_i = a_i \cdot b_i$.


Let $I = [-k/2,k/2]$ and $B,C$ sets in $[-n/2,n/2]$ for $n$ much larger than $k$. We define vector $1_B$ to denote the vector such that $(1_B)_i = 1$ if $i\in B$ and $(1_B)_i = 0$ otherwise. We want to approximate $(1_B * 1_C) \odot 1_I$.

\textbf{idea}:

Look at $( 1_B \odot f ) * ( 1_C \odot g )$, the $i$-th entry of which is
\begin{align*}
\sum_{j=-n/2}^{n/2} (1_B)_j \cdot f_j \cdot (1_C)_{i-j} \cdot g_{i-j}.	
\end{align*}
One easy fact we know is
\begin{fact}
Given four vectors $a,b,c,d$, we have
\begin{align*}
(a \odot b) * (c \odot d) = (a * c) \odot ( b * d )
\end{align*}
\end{fact}
\begin{proof}
For each $i$, we have
\begin{align*}
\LHS = & ~ ( (a \odot b) * (c \odot d) )_i \\
= & ~ \sum_j (a \odot b)_j \cdot ( c \odot d )_{i-j} \\
= & ~ \sum_j a_j b_j c_{i-j} d_{i-j} \\
= & ~ ??? \\
= & ~ ( \sum_j a_j c_{i-j} ) \cdot ( \sum_j b_j d_{i-j} ) \\
= & ~ ( a * c )_i \cdot ( b * d )_i \\
= & ~ ( ( a * c ) \odot ( b * d ) )_i \\
= & ~ \RHS
\end{align*}
\end{proof}

Using the above fact, we have
\begin{align*}
( 1_B \odot f ) * ( 1_C \odot g ) = (1_B * 1_C) \odot (f * g). %(1_B * 1_C) \odot I
\end{align*}

If the following two things hold,

\begin{itemize}
\item For $|i| > k \log^c k$, $\sum_{j \in [-n/2,n/2] } f_j g_{i-j} < 1/(2k^2)$.
\item For $|i| \leq k/2$ and all $j$, $f_j g_{i-j} \geq 1/k$, (-> $(f*g)_i \geq 1$)  
\end{itemize}
(\Zhao{it means in \cite{hikp12a} }, $n/(2B) = k$; $f * g \approx I$)
then we are done. 
Can we find such functions $f$ and $g$? Possibly for $f$ to be the discrete Gaussian distribution, and $g$ to be the indicator of $I$, that would work.


%roughly $m^{1-\delta}$ subproblems, each problem has three sets $B,C,I$, $|B| = |C| = |I| = m^{\delta}$.

Originally, the way how they solved it, is using additive combinatorics.
We don't use additive combinatorics.

(Zhao : i don't know how to implement this step.)The running time is $m^{2-O(\delta)}$, our goal is $m^{2-\delta}$

Compute $(1_B * 1_C) \odot 1_I$, 
computing $(1_B * 1_C)$ either takes $n \log n$ time or $k^2$ time. $|B|=|C|=|I|=k$.

$f * g$ approximate $1_I$ ($f * g$ Fourier filter function)

\begin{comment}
1)
if $|i| > 1 \cdot n$, $(f * g)_i \in +/- \delta$
if $|i| \in \alpha/2, 1$, $(f * g)_i \in [0,1] $
if $|i| < \alpha/2 \cdot n$, $(f * g)_i \in 1 +/- \delta$ 

2)
if $i \leq 1 \cdot n$, $(1_I)_i = 1$
else $(1_I)_i = 0$

\end{comment}
$(1_B * 1_C) \odot 1_I 
\approx 
(1_B * 1_C) \odot (f * g) 
\approx
(1_B \odot f) * (1_C \odot g)$,
(location Fourier set query has the definition of $f$ and $g$)

\subsection{Important tricks used in previous sparse FT paper}

\subsubsection{Subsampled FFT}
In \cite{hikp12b}, it mentioned a trick called ``subsampled FFT''. Suppose we have a vector $x \in \C^n$ and a parameter $B$ dividing $n$, and would like to compute $\wh{y}_i = \wh{x}_{ i ( n / B ) }$ for $i \in [B]$.

\begin{claim}[Claim 3.7 in \cite{hikp12b}]
Let vector $y \in \C^B$ be defined as follows : for each $i \in [B]$, $y_i = \sum_{j=0}^{n/B-1} x_{i+ B j}$. Let $\wh{y}$ denote the Fourier transform of $y$.

Therefore $\wh{y}$ can be computed in $O( | \supp(x) | + B \log B )$ time.
\end{claim}
\begin{proof}
Let $\omega = e^{2\pi \i / n}$
We have
\begin{align*}
\wh{x}_{ i (n/B) } = & ~ \sum_{j = 0}^{n-1} x_j \omega^{ij (n/B)} & \text{~by~} \wh{x} = \textsc{FT}(x) \\
= & ~ \sum_{a = 0}^{B-1} \sum_{j = 0}^{n/B-1} x_{ B j + a } \omega^{i (B j + a) n/B} \\
= & ~ \sum_{a = 0}^{B-1} \sum_{j = 0}^{n/B-1} x_{ B j + a } \omega^{i a n / B} & \text{~by~} \omega^{ijn} = 1 \\
= & ~ \sum_{a = 0}^{B-1} y_a \omega^{i a n / B} & \text{~by~} \sum_{j = 0}^{n/B-1} x_{ B j + a } = y_a \\
= & ~ \wh{y}_i . & \text{~by~} \wh{y} = \textsc{FT}(y)
\end{align*}
\end{proof}

\subsubsection{Semi-equispaced Fourier Transform}

See Section 12, page 42 of \url{https://theory.epfl.ch/kapralov/papers/fourier-measurements.pdf}.

\begin{algorithm}[h]\caption{}
\begin{algorithmic}[1]
\Procedure{\textsc{SemiEquispaceFFT}}{$x,c$}
	\State Round $k$ up to a factor of $n$
	\State $G, \wh{G'} \leftarrow \textsc{Filters}(n,k,c)$
	\State $y_i \leftarrow \frac{1}{ \sqrt{n} } ( x * G )_{i n / 2k} $ for $i \in [2k]$
	\State $\wh{y} \leftarrow \textsc{FFT}(y)$
	\State $\wh{x}_i' \leftarrow \wh{y}_i$ for $|i| \leq k / 2$
	\State \Return $\wh{x}'$
\EndProcedure
\end{algorithmic}
\end{algorithm}


\subsection{Filter function}


\subsubsection{Continuous version}
We define rect and sinc function as follows:
\begin{definition}[page 12 in \cite{ckps16}]
\begin{align*}
\sinc (t) = \frac{ \sin ( \pi t ) }{ \pi t }
\end{align*}
\end{definition}

\begin{fact}[continuous version, fact 3.3 in \cite{ckps16}]
We define
\begin{align*}
\rect_s(t) = 
\begin{cases}
1, & \text{~if~} |t| \leq \frac{s}{2}; \\
0, & \text{~otherwise}.
\end{cases}
\end{align*}
Then Fourier transform a of $\rect_s(t)$ is $\wh{\rect_s}(f) = \frac{ \sin( \pi f s ) }{ \pi f s} = \sinc(f s)$.
\end{fact}

Note that \cite{ckps16} used continuous filter function $G(t), \wh{G}(f)$ \footnote{\url{https://arxiv.org/pdf/1609.01361.pdf}, page 79.}. Here we use discrete filter function,
\begin{definition}[continuous version, definition C.11 in \cite{ckps16}]
\begin{align*}
G(t) = & ~ b_0 \cdot ( \rect_{s_1} ( t ) )^{* l} \cdot \sinc ( s_2 t ), \\
\wh{G}_f = & ~ b_0 \cdot ( \sinc ( s_1 f ) )^{\cdot l} * \rect_{s_2} ( f ).
\end{align*}
\end{definition}

\subsubsection{Discrete version}

We can make the discrete version,
\begin{definition}[discrete version]
We define
\begin{align*}
G_i = & ~ b_0 \cdot ( \rect_{s_1} ( i ) )^{* l} \cdot \sinc ( s_2 i ), \forall i \in [n] \\
\wh{G}_i = & ~ b_0 \cdot ( \sinc ( s_1 i ) )^{\cdot l} * \rect_{s_2} ( i ), \forall i \in [n].
\end{align*}
\end{definition}

\begin{lemma} [Properties of the $\sinc$ function, Appendix C in \cite{ckps16}] \label{lem:sinc_property}
% \begin{enumerate}
% \item $\forall t \in \R, 1 - \frac{(\pi t)^2}{3!} \leq \sinc(t) \leq 1$.
% \item $\forall |t| \leq 1.2 / \pi, \sinc(t) \leq 1 - t^2 / 8$. 
% Looks like the above two are not useful here
% \item 
\begin{align*}
\forall |t| > 1.2 / \pi, |\sinc(t)| \leq \frac{1}{\pi |t|}.
\end{align*}
% \end{enumerate}
\end{lemma}

\newpage
% \Zhao{I think we need to compute the following thing. Zhengyu, can you do that?}
\Zhengyu{I tried to adapt the following proof from \cite{ckps16}. Please check if it looks OK.}
\begin{claim}
For each $|i| \leq k/2$, we have
\begin{align*}
\wh{G}_i \in [ 1 - \delta, 1].
\end{align*}
For each $|i| \geq k \log^c k$, we have
\begin{align*}
\wh{G}_i \in [-\delta, \delta].
\end{align*}
\end{claim}

\begin{proof}
By definition of $\wh{G}$, we can rewrite
\begin{align*}
\wh{G}_i = & ~ \sum_{j=1}^n b_0 \cdot ( \sinc (s_1 j) )^{l} \cdot \rect_{s_2} (i - j) \\
= & ~ \sum_{ j \in [i-s_2/2, i+s_2/2] } b_0 \cdot ( \sinc (s_1 j) )^{l}
\end{align*}
The choice for $s_1$, $s_2$, $l$ ($l$ is even number) should be
\begin{align*}
s_1 = \frac{2B}{\alpha n}, ~~~ s_2 = \frac{n}{4B}, ~~~ l = \Omega( \log (k/\delta) )
\end{align*}
For $\alpha$, the choice should $[1/10,9/10]$. 
For $B$, the choice should be $\Theta(n/k)$, since $\Theta(n/B) = k$.
For $b_0$, the choice should be $\Theta(s_1 \sqrt{l}) = \Theta(B \sqrt{l}/ (\alpha n ))$ since we hope $\wh{G}(0) =1$.
Let $s_1 = \beta_1 / k$, and by definition of $s_1$ we have $\beta_1 = \Theta(1)$.
We require that $s_2 \geq (\frac{2}{\beta_1} + 1) k$. In addition, we require $\frac{s_1 s_2}{2}$ is an integer, in order to make subsequent arguments go through.
\Zhengyu{Please check if the above two additional assumptions make any trouble.}

We first prove that 
\begin{align}	
\sum_{j = k/\beta_1}^{\infty} b_0 (\sinc(s_1 j))^l \leq \delta / 2, \label{eq:sinc_tail_sum}
\end{align}

which follows from
\begin{align*}
\sum_{j = k/\beta_1}^{\infty} b_0 (\sinc(s_1 j))^l = & ~ b_0 \sum_{j = k/\beta_1}^{\infty} (\sinc(\beta_1 j / k))^l \\
\leq & ~ b_0 \sum_{j = k/\beta_1}^{\infty} \frac{1}{(\pi \beta_1 j / k)^l} \\
= & ~ b_0 \pi^{-1} \sum_{t = 1}^{\infty} \sum_{j = t k /\beta_1}^{(t+1) 
\frac{k}{\beta_1} - 1} \frac{1}{(\beta_1 j / k)^l} \\
\leq & ~ b_0 \pi^{-l} \sum_{t = 1}^{\infty} \left( \frac{k}{\beta_1} \cdot \frac{1}{t^{l}} \right) \\
= & ~ b_0 \pi^{-l} \cdot \frac{k}{\beta_1} \cdot \sum_{t = 1}^{\infty} \frac{1}{t^{l}} \\
\leq & ~ \delta / 2,
\end{align*}

where the second step follows from Lemma~\ref{lem:sinc_property}, and the last step follows by $l = \Omega(\log (k / \delta))$ and our choice of $b_0 = \Theta(\frac{\sqrt{l}}{k})$.

\noindent
(1) For $|i| \leq k/2$. We will first prove that $\wh{G}_i \leq \wh{G}_0$.
We assume that $0 < i \leq k/2$. The case that $-k/2 \leq i < 0$ is symmetric.

\begin{align*}
\wh{G}_0 - \wh{G}_i = & ~ \sum_{j=-s_2/2}^{s_2/2} b_0 \cdot ( \sinc (s_1 j) )^{l} - \sum_{j = i-s_2/2}^{i+s_2/2} b_0 \cdot ( \sinc (s_1 j) )^{l} \\
= & ~ \sum_{j=-s_2/2}^{i-s_2/2} b_0 \cdot ( \sinc (s_1 j) )^{l} - \sum_{j = s_2/2}^{i+s_2/2} b_0 \cdot ( \sinc (s_1 j) )^{l} \\
= & ~ \sum_{t = 0}^{i} b_0 \cdot ( \sinc (s_1 (t - s_2 / 2)) )^{l} - \sum_{t=0}^{i} b_0 \cdot ( \sinc (s_1 (t + s_2 / 2)) )^{l} \\
= & ~ \sum_{t = 0}^{i} b_0 \cdot ( \sinc (s_1 (-t + s_2 / 2)) )^{l} - \sum_{t=0}^{i} b_0 \cdot ( \sinc (s_1 (t + s_2 / 2)) )^{l} \\
= & ~ b_0 \sum_{t = 0}^{i} \left( ( \sinc (s_1 (-t + s_2 / 2)) )^{l} - ( \sinc (s_1 (t + s_2 / 2)) )^{l} \right) \\
= & ~ b_0 \sum_{t = 0}^{i} \left( \frac{|\sin(\pi s_1 s_2 / 2 - \pi s_1 t)|^l}{(\pi s_1 (-t + s_2/2))^l} - \frac{|\sin(\pi s_1 s_2 / 2 + \pi s_1 t)|^l}{(\pi s_1 (t + s_2/2))^l} \right) \\
= & ~ b_0 \sum_{t=0}^{i} \frac{|\sin(\pi s_1 t)|^l}{(\pi s_1)^l} \left( \frac{1}{(-t+s_2/2)^l} - \frac{1}{(t+s_2/2)^l} \right) \\
\geq & ~ 0,
\end{align*}

where the forth step follows by the function $\sinc(\cdot )^l$ is an even function because $l$ is an even integer, the seventh step follows by $\frac{s_1s_2}{2}$ is an integer, and the last steps follows by $|-t + s_2/2| \leq |t + s_2/2|$. By our choice of $b_0$, we have $\wh{G}_0 = 1$. Therefore, $\wh{G}_i \leq 1$.

Now we will prove that $\wh{G}_i \geq 1 - \delta$.
Note that by our assumption that $s_2 \geq (\frac{2}{\beta_1}+1)k$, we have $\frac{s_2}{2} - \frac{k}{2} \geq \frac{k}{\beta_1}$. 
For $|i| \leq \frac{k}{2}$, we have $i-\frac{s_2}{2}-1 \leq \frac{k}{2} - \frac{s_2}{2} -1 \leq -\frac{k}{\beta_1}$ and $i+\frac{s_2}{2}+1 \geq \frac{k}{2} + \frac{s_2}{2} + 1 \geq \frac{k}{\beta_1}$.
Therefore,

\begin{align*}
\wh{G}_i = & ~ \sum_{j=-\infty}^{\infty} b_0 \cdot ( \sinc (s_1 j) )^{l} - \sum_{j=-\infty}^{i - s_2/2 - 1} b_0 \cdot ( \sinc (s_1 j) )^{l} - \sum_{j = i + s_2/2 + 1}^{\infty} b_0 \cdot ( \sinc (s_1 j) )^{l} \\
\geq & ~ \sum_{j=-k/2}^{k/2} b_0 \cdot ( \sinc (s_1 j) )^{l} - \sum_{j=-\infty}^{-k / \beta_1} b_0 \cdot ( \sinc (s_1 j) )^{l} - \sum_{j = k / \beta_1}^{\infty} b_0 \cdot ( \sinc (s_1 j) )^{l} \\
= & ~ 1 - 2 \sum_{j = k / \beta_1}^{\infty} b_0 \cdot ( \sinc (s_1 j) )^{l} \\
\geq & ~ 1 - \delta,
\end{align*}

where the last step follows from \eqref{eq:sinc_tail_sum}.

\noindent
(2) For $|i| \geq k\log^c k$, we can bound $\wh{G}_i$:
\begin{align*}
\wh{G}_i = & ~ b_0 \sum_{j = i-s_2/2}^{i+s_2/2} (\sinc(\beta_1 j / k))^l \\
\leq & ~ b_0 \sum_{j = k / \beta_1}^{\infty} (\sinc(\beta_1 j / k))^l \\
< & ~ \delta,
\end{align*}
where the second step follows by $s_2 = \Theta(k)$ and $|i| \geq k \log^c k$ so that $i - s_2/2 \geq k / \beta_1$, and the third step follows by \eqref{eq:sinc_tail_sum}.

\end{proof}


\subsection{New filter}

\Zhao{Billy, can you write down the property of the filter (you think will work), first? Then we can discuss how to construct the filter.}


\begin{comment}
Let $I$ denote a continuous size $k$ set. Let $B$, $C$ denote two $k$-sparse vectors, let $G$ denote the Gaussian filter, and $P$ denote the rectangular filter. Roughly speaking $G * P \approx I$. We define vector $z$ as follows:
\begin{align*}
z = ( B \cdot G ) * ( C \cdot P )
\end{align*}
We want to prove two things : \\
1. If $|i| < k/2$, then $z_i$ is large \\
2. If $|i| > k$, then $z_i$ is small

One fact we know is
\begin{align*}
( B \cdot G ) * ( C \cdot P ) = (B * C) \cdot ( G * P ).
\end{align*}
\end{comment}


==> warmup.tex <==
\section{$O(k \log n)$ measurements for $k = O(\log n)$}\label{sec:warmup}
We first discuss a measurement reuse idea that leads us to a sparse recovery algorithm (Algorithm~\ref{alg:fourier_sparse_recovery_k_logn}) taking $O(k \log n)$ measurements for $k = O(\log n)$.
We set $H = 5$, and let ${\cal T} = \{{\cal T}^{(1)}, \ldots, {\cal T}^{(H)}\}$, where each ${\cal T}^{(h)}$ is a list of $O(k \log n)$ i.i.d. elements in $[p]^d$.
Note that ${\cal T}^{(1)}, \ldots, {\cal T}^{(H)}$ are independent.
In our sparse Fourier recovery algorithm, we will measure $x_t$ for all $t \in {\cal T}$.


In a nutshell, our approach finely discretizes the space of possible trajectories the algorithm could evolve, and carefully argues about the correctness of the algorithm by avoiding the intractable union-bound over all trajectories.

\paragraph{Recovery algorithm.} The recovery algorithm proceeds in $\log R^* - H + 1$ iterations, where each iteration (except the last iteration) the goal is to reduce the upper bound of $\ell_\infty$ norm of the residual signal by half. 
Initially, the upper bound is $R^*$.
It is important to note that we use the same measurements ${\cal T} = \{{\cal T}^{(1)}, \ldots, {\cal T}^{(H)}\}$ in all of these $\log R^* - H + 1$ iterations.

In the following, we will describe one iteration of the recovery algorithm. 
Let $y \in \C^{[p]^d}$ denote the sparse vector recovered so far, and let the upper bound of $\|\wh{x} - y\|_\infty$ be $2 \nu$. 
Running the \textsc{LinfinityReduce} procedure $H$ times where in the $h$-th time we use measurements in ${\cal T}^{(h)}$, we obtain a $O(k)$-sparse $z$ such that with probability $1 - 1 / \poly(n)$, $\|\wh{x} - y - z\|_\infty \leq 2^{1-H} \nu \leq 0.1 \nu$ (we call such $z$ a desirable output by the \textsc{LinfinityReduce} procedure).
Instead of taking $y+z$ as our newly recovered sparse signal, for each $f \in \supp(y+z)$, we project $y_f+z_f$ to the nearst points in $\mathcal{G}_{0.6 \nu}:= \{0.6 \nu (x + y \i): x,y \in \Z \}$ and assign to $y'_f$, where $y'$ denotes our newly recovered sparse signal.
For all $f \not\in \supp(y+z)$, we let $y'_f = 0$.

To simplify our exposition, here we introduce some notations.
We call $\mathcal{G}_{0.6 \nu}$ a grid of side length $0.6 \nu$, and we generalize the definition to any side length.
Namely, for any $r_g > 0$, let grid $\mathcal{G}_{r_g}:= \{r_g(x + y \i): x,y \in \Z \}$.
Moreover, we define $\Pi_{r_g}: \C \rightarrow \mathcal{G}_{r_g}$ to be the mapping that maps any element in $\C$ to the nearest element in $\mathcal{G}_{r_g}$.
Now we can write $y'$ as
\begin{align*}
y'_f = 
\begin{cases} 
  \Pi_{0.6 \nu}(y_f + z_f), & \text{~if~} f \in \supp(y+z); \\ 
  0, & \text{~if~} f \not\in \supp(y+z).
\end{cases} 
\end{align*}

At the end of each iteration, we assign $y'$ to $y$, and shrink $\nu$ by half. In the last iteration, we will not compute $y'$, instead we output $y+z$. 
We present the algorithm in Algorithm~\ref{alg:fourier_sparse_recovery_k_logn}.

\begin{algorithm}[!t]\caption{Fourier sparse recovery by projection, $O(k \log n)$ measurements when $k = O(\log n)$}\label{alg:fourier_sparse_recovery_k_logn}
\begin{algorithmic}[1]
\Procedure{\textsc{FourierSparseRecoveryByProjection}}{$x,n,k,\mu,R^*$} \Comment{Section~\ref{sec:warmup}} 
  \State {\bf Require} that $\mu = \frac{1}{\sqrt{k}} \|\wh{x}_{-k}\|_2$ and $R^* \geq \|\wh{x}\|_\infty\ / \mu$ 
  \State $H \leftarrow 5$, $\nu \leftarrow \mu R^* / 2$, ~$y \leftarrow \vec 0$ \Comment{$y \in \C^{[p]^d}$ refers to the sparse vector recovered so far}
  \State Let ${\cal T} = \{ {\cal T}^{(1)}, \cdots, {\cal T}^{(H)} \}$ where each ${\cal T}^{(h)}$ is a list of i.i.d. uniform samples in $[p]^d$ 
  \While {{\bf true}} 
    \State $\nu' \leftarrow 2^{1-H} \nu$
    \State Use $\{x_t\}_{t\in \mathcal{T}}$ to run the \textsc{LinfinityReduce} procedure (in Lemma~\ref{lem:locate_and_estimate_informal}) $H$ times (use samples in ${\cal T}^{(h)}$ for each $h\in [H]$ ), and finally it finds $z$ so that $\|\wh{x} - y - z\|_\infty \leq \nu'$ 
    \State{{\bf if} {$\nu' \leq \mu$} } {\bf then} \Return $y+z$ \Comment{We found the solution}
    \State $y' \leftarrow \vec 0$
    \For{$f \in \supp(y+z)$}
      \State $y'_f \leftarrow \Pi_{0.6 \nu}(y_f + z_f)$ \Comment{We want $\|\wh{x} - y' \|_\infty \leq \nu$ and the depend-}
    \EndFor \Comment{ence between $y'$ and $\mathcal{T}$ is under control~~~}
    \State $y \leftarrow y'$, $\nu \leftarrow \nu / 2$
  \EndWhile
\EndProcedure
\end{algorithmic}
\end{algorithm}

\paragraph{Analysis.} We analyze $y'$ conditioned on the event that $\|\wh{x} - y - z\|_\infty \leq 0.1 \nu$ (i.e. $z$ is a desirable output by the \textsc{LinfinityReduce} procedure, which happens with probability $1 - 1 / \poly(n)$).
We will prove that $y'$ has two desirable properties: (1) $\|\wh{x} - y'\|_\infty \leq \nu$; (2) the dependence between $y'$ and our measurements ${\cal T}$ is under control so that after taking $y'$ as newly recovered sparse signal, subsequent executions of the \textsc{LinfinityReduce} procedure with measurements ${\cal T}$ still work with good probability. 
Property (1) follows from triangle inequality and the fact that $\|\wh{x} - (y+z)\|_\infty \leq 0.1 \nu$ and $\|(y+z) - y'\|_\infty \leq 0.6 \nu$.
We now elaborate on property (2). 
We can prove that for any $f \in [p]^d$, 
\begin{align*}
y'_f \in \big\{\Pi_{0.6\nu}(\wh{x}_f+0.1\nu(\alpha+ \beta\i)): \alpha, \beta \in \{-1, 1\} \big\}.
\end{align*}
Let $S$ denote top $26 k$ coordinates (in absolute value) of $\wh{x}$.
We can further prove that for any $f \in \ov{S}$, $y'_f =0$.
Therefore, the total number of possible $y'$ is upper bounded by $4^{|S|} = 4^{O(k)}$.
If $k = O(\log n)$, we can afford union bounding all $4^{O(k)} = \poly(n)$ possible $y'$, and prove that with probability $1 - 1 / \poly(n)$ for all possible value of $y'$ if we take $y'$ as our newly recovered sparse signal then in the next iteration the \textsc{LinfinityReduce} procedure with measurements ${\cal T}$ gives us a desirable output.

\paragraph{Sufficient event.}
More rigorously, we formulate the event that guarantees successful execution of Algorithm~\ref{alg:fourier_sparse_recovery_k_logn}.
Let ${\cal E}_1$ be the event that for all $O(\log R^*)$ possible values of $\nu \in \{ \mu \frac{ R^*}{2}, \mu \frac{ R^*}{4}, \ldots, \mu 2^{H-1} \}$,
for all possible vector $y$ where $y_f = 0$ for $f \in \ov{S}$ and $y_f \in \{ \Pi_{0.6 \nu} (\wh{x}_f + 0.1 \nu(\alpha + \beta \i)): \alpha, \beta \in \{-1, 1\} \}$ for $f \in S$ (we also need to include the case that $y = \vec 0$ for the success of the first iteration), 
running the \textsc{LinfinityReduce} procedure (in Lemma~\ref{lem:locate_and_estimate_informal}) $H$ times (where in the $h$-th time measurements $\{x_t\}_{t \in {\cal T}^{(h)}}$ are used to reduce the error from $2^{2-h} \nu$ to $2^{1-h} \nu$) finally gives $z$ so that $\|\wh{x} - y - z\|_\infty \leq 2^{1-H} \nu$.
The randomness of ${\cal E}_1$ comes from ${\cal T} = \{ {\cal T}^{(1)}, \ldots, {\cal T}^{(H)} \}$.

First, event ${\cal E}_1$ happens with probability $1 - 1 / \poly(n)$. This is because there are $4^{O(k)} \log R^*$ possible combinations of $\nu$ and $y$ to union bound, and each has failure probability at most $1 / \poly(n)$.
For $k = O(\log n)$, and any $R^* < 2 ^{n^{100}}$ this gives the desired result.
Second, conditioned on event ${\cal E}_1$ happens, Algorithm~\ref{alg:fourier_sparse_recovery_k_logn} gives correct output.
This can be proved by a mathematical induction that in the $t$-th iteration of the while-true loop in Algorithm~\ref{alg:fourier_sparse_recovery_k_logn}, $\|\wh{x} - y\|_\infty \leq 2^{-t} \mu R^*$.
